Robust and Resource Efficient Identification of Two Hidden Layer Neural Networks

We address the structure identification and the uniform approximation of two fully nonlinear layer neural networks of the type $f(x)=1^T h(B^T g(A^T x))$ on $\mathbb R^d$ from a small number of query samples. We approach the problem by sampling actively finite difference approximations to Hessians of the network. Gathering several approximate Hessians allows reliably to approximate the matrix subspace $\mathcal W$ spanned by symmetric tensors $a_1 \otimes a_1 ,\dots,a_{m_0}\otimes a_{m_0}$ formed by weights of the first layer together with the entangled symmetric tensors $v_1 \otimes v_1 ,\dots,v_{m_1}\otimes v_{m_1}$, formed by suitable combinations of the weights of the first and second layer as $v_\ell=A G_0 b_\ell/\|A G_0 b_\ell\|_2$, $\ell \in [m_1]$, for a diagonal matrix $G_0$ depending on the activation functions of the first layer. The identification of the 1-rank symmetric tensors within $\mathcal W$ is then performed by the solution of a robust nonlinear program. We provide guarantees of stable recovery under a posteriori verifiable conditions. We further address the correct attribution of approximate weights to the first or second layer. By using a suitably adapted gradient descent iteration, it is possible then to estimate, up to intrinsic symmetries, the shifts of the activations functions of the first layer and compute exactly the matrix $G_0$. Our method of identification of the weights of the network is fully constructive, with quantifiable sample complexity, and therefore contributes to dwindle the black-box nature of the network training phase. We corroborate our theoretical results by extensive numerical experiments.

==> sections/matrix_subspace/subsection1_whatever.tex <==

\subsection{Approximating $L$ by $L_{PCA}$}
Lets assume we have $m_x \in \mathbb{N}$ different points $\ve{x}_1, \dots, \ve{x}_{m_x} \in \mathbb{R}^d$ and  $H_f(\ve{x}_1), ..., H_f(\ve{x}_{m_x}) \in \mathbb{R}^{d\times d}$ are known. Now we can construct the matrix $M$ given by
\begin{align}\label{defM}
\ma{M} := \left( \opvec(H_f(\ve{x}_{1}) \middle|... \middle| \opvec(H_f(\ve{x}_{m_x}))\right) \in \mathbb{R}^{d^2 \times m_x}.
\end{align} 
If $m_x$ is large and the $\ve{x}_i$ are well distributed, the column space $\operatorname{range}(M)$ of $\ma{M}$ will eventually come very close the space spanned by the vectorized Hessians. To make sure the points $\ve{x}_1, \dots, \ve{x}_{m_x}$ are well distributed, we will draw from the uniform distribution on the unit sphere 
\begin{align}
\mathbb{S}^{d-1} := \set{x \in \mathbb{R}^d \given \norm{x}_2 = 1 }.
\end{align}
We get the approximation $L_{PCA} \approx L$ by setting $L_{PCA}$ to the column space of the first $m+m_1$ left singular vectors of $M$.  To be precise, let 
\begin{align}\label{svd:M}      
\ma{M} &= \begin{pmatrix}\ma{U}_1 & \ma{U}_2\end{pmatrix}
\begin{pmatrix}\ma{\Sigma}_1 &0 &0\\ 0 & \ma{\Sigma}_2 &0\end{pmatrix}
\begin{pmatrix}\ma{V}^T_1 \\ \ma{V}^T_2\end{pmatrix}
\end{align}
be the singular value decomposition of $M$, where $U_1 = (u_1|\dots|u_{m+m_1}) \in \mathbb{R}^{d^2\times (m+m_1)}$. Then we set $L_{PCA}$ to the column space $\operatorname{range}(U_1)$ of $U_1$. This procedure is summarized in Algorithm \ref{alg:dimred}.
\begin{rem}
	The space $L\subset \mathbb{R}^{d\times d}$ is a subspace of matrices, while $L_{PCA} \subset \mathbb{R}^{d^2}$ is a vector subspace. We are aware that this might cause confusion and will address our representation of matrix subspaces at the beginning of Section \ref{section:concMain}.
\end{rem}

\begin{algorithm}
	\KwIn{$f \in \mathcal{F}_d(m_1, m)$}
	\Parameter{$m_x$}
	\KwOut{$L_{PCA}$}    
	\Begin{
		Sample $x_1,\dots, x_{m_x}$ uniformly from $\mathbb{S}^{d-1}$\;
		$M \leftarrow \left(\opvec(H_f(x_1)) | \dots | \opvec(H_f(x_{m_x})) \right)$\;
		$\begin{pmatrix} U_1 & U_2 \end{pmatrix}\Sigma V^T \leftarrow SVD(M)$\;
		$L_{PCA}\leftarrow \operatorname{range}(u_1 | \dots | u_{m+m_1})$\;
	}
	\caption{Dimension reduction on the span of the Hessians}\label{alg:dimred} 
\end{algorithm}
\iffalse
The algorithm has to be seen as a general framework. It can be separated into two steps. First, we evaluate the Hessians such that $\operatorname{range}(M)$ is a rich space, hopefully containing enough information to reconstruct the directions $a_1,\dots, a_m,v_1, \dots, v_\ell$. This clearly depends on the choice of our distribution. Drawing $x_1, \dots, x_{m_x}$ uniformly from the sphere has several benefits which will be discussed in the next section. Nevertheless, it is important to address that we do not claim that this distribution is optimal. Finding a better way to sample the Hessians depending on the structure of the problem is not a focus of this thesis, but we will demonstrate some ideas regarding this topic in the numerical part. One simple example is to change the radius of the sphere, which can have a large impact on the final result (see chapter \ref{chapter:numerics}).
\\
The second step consists of a dimensionality reduction based on the singular value decomposition of $M$.
Picking the first $m+m_1$ singular vectors is a natural decision, we simply choose to approximate the $m+m_1$ dimensional space $L$ by a $m+m_1$ dimensional space. Deviating from this choice would automatically lead to a difference between $L$ and $L_{PCA}$.\\
\fi

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%START BETA%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\input{./tex/chapter2/beta.tex}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%END BETA%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

==> sections/matrix_subspace/subsection2_concentration.tex <==
\subsection{Concentration of $L_{PCA}$ around $L$}\label{section:concMain}
\emph{Explain how $L$ has to be understand, previous explanation} \color{red} $\langle$ deleted $\rangle$ \\\\ \color{black} 
Let $P_L$ be the orthogonal projection onto $L$, and suppose $\ve{x}_1,..., \ve{x}_{m_x}$ are drawn uniformly from the unit sphere $\mathbb{S}^{d-1}$ at random. According to  Algorithm \ref{alg:dimred}, we construct $L_{PCA}$ as the span of the first $m+m_1$ left singular vectors of the matrix
\begin{align}\label{def_M}
M = \left[ \opvec(H_f(\ve{x}_1))\middle| ...\middle| \opvec(H_f(\ve{x}_{m_x}))\right] \in \mathbb{R}^{d^2 \times m_x}.
\end{align}
We further denote 
\begin{align}\label{def_hatM}
\hat{M} = \left[  \opvec(P_L H_f(\ve{x}_1))\middle| ...\middle|  \opvec(P_L H_f(\ve{x}_{m_x}))\right] \in \mathbb{R}^{d^2 \times m_x}
\end{align}
and set $\hat{L} = \operatorname{range}(\hat{M})$.

\iffalse
Note that $\hat{L} \subseteq L^{vec}$ (cf. \ref{def:Lvec}), therefore 
\begin{align*}\operatorname{dim}(\hat{L}) \leq \operatorname{dim}(L^{vec}) \leq m+m_1. \end{align*}
We want to show that $L_{PCA}$ concentrates around $L^{vec}$. This will be done in two steps. First, we develop upper bounds for the distance of $L_{PCA}$ and $\hat{L}$. Second, we show that $\hat{L} = L^{vec}$ if $L_{PCA}$ and $\hat{L}$ are close enough. Since the algorithm acts upon random matrices, we aim for bounds that hold with high probability. In (\ref{dim_span_hessians}) we already pointed out that 
\begin{align*}
\operatorname{dim}\opspan \set{H_f(\ve{x}) \given \ve{x} \in \mathbb{R}^d} \leq \frac{m(m+1)}{2}.
\end{align*}
It is reasonable to assume that the dimension of the span does not change when we restrict $\ve{x}$ to the unit sphere $x \in \mathbb{S}^{d-1}$. However, the dimension of the span also depends on the rank of $\ma{G}_x \ma{B} \ma{S}_x \ma{B}^T \ma{G}_x + \ma{T}_x \in \mathbb{R}^{m\times m}$ (cf. \ref{hessian_matrep}). To show the concentration, we need to make sure that the rank of $M$ is sufficiently large. Due to (\ref{span_mixed}), all columns of $M$ lie in the space spanned by $ \opvec(\ve{a}_j \otimes \ve{a}_i + \ve{a}_i \otimes \ve{a}_j), 1\leq i\leq j\leq m$. One assumption could be, that, by sampling enough vectors $\opvec(H_f(\ve{x}_1)), \dots ,\opvec(H_f(\ve{x}_{m_x}))$, we will get the space 
\begin{align*}
\opspan \set{\opvec(H_f(\ve{x}_n))  \given n= 1,\dots, m_x} \cong \opspan \left\lbrace \opvec\left( \ve{a}_j \otimes \ve{a}_i + \ve{a}_i \otimes \ve{a}_j\right)\middle|  1 \leq i \leq j \leq m\right\rbrace. 
\end{align*}
This is equivalent to $\oprank(\ma{M}) = m(m+1)/2$ for $m_x$ large enough, or $\sigma_{\frac{m(m+1)}{2}}(\ma{M}) > 0$. Here $\sigma_k(\ma{M})$ denotes the $k$-th singular value of $\ma{M}$. Note that we have 
\begin{align}\label{singular_expression}
\sigma_k(\ma{M}) = \sqrt{\sigma_k(\ma{M}\ma{M}^T)}, \,\text{ for } k = 1,\dots, \max\left\lbrace m_x, d^2\right\rbrace.
\end{align}
Additionally 
\begin{align}
\ma{M}\ma{M}^T = \sum_{i=1}^{m_x} \opvec(H_f(\ve{x}_i))^{\otimes 2}\in \mathbb{R}^{d^2 \times d^2}, 
\end{align}
which is a sum of independent matrices. Since $\opvec(H_f(\ve{x_i}))$ is bounded, $\opvec(H_f(\ve{x}_i))$ has finite second moments and by the law of large numbers  
\begin{align*}
\frac{1}{m_x}\sum_{i=1}^{m_x} \opvec(H_f(\ve{x}_i))^{\otimes 2} \to \mathbb{E}_{X \sim \mu_{\mathbb{S}^{d-1}}}\left[\opvec(H_f(\ve{X}))^{\otimes 2} \right]
\end{align*}
for $m_x \to \infty$. Therefore, 
\begin{align*}
\sigma_k(\ma{M}) \approx \sqrt{m_x \sigma_k\left( \mathbb{E}\left[ \opvec(H_f(\ve{X}))^{\otimes 2} \right]\right)} 
\end{align*}
for $m_x$ large. The quality of this approximation depends on the number of samples $m_x$ and the deviation of $\opvec(H_f(\ve{X}))^{\otimes 2}$
from its mean. We want to show that the Hessians concentrate around a space of dimension $m+m_1$. If we want to be able to construct the full space, we need 
$\left(\mathbb{E}_{\mu_{\mathbb{S}^{d-1}}}\left[ \opvec(H_f(X))^{\otimes 2} \right]\right)$ to have at least rank $m+m_1$. So for our analysis we formulate the following assumption:
\fi
\begin{assump}\label{assump:lowersvbound}
	The $m+m_1$-th singular value of
	\begin{align*}
	\mathbb{E}_{\mu_{\mathbb{S}^{d-1}}} \left[ \opvec(H_f(X))^{\otimes 2} \right] = \int_{\mathbb{S}^{d-1}}\opvec(H_f(x))^{\otimes 2} d\mu_{\mathbb{S}^{d-1}}(x)
	\end{align*}
	is well separated from $0$, i.e. there is an $\alpha > 0$ such that
	\begin{align}\label{alpha_bound}
	\sigma_{m+m_1}\left(\mathbb{E}_{\mu_{\mathbb{S}^{d-1}}}\left[ \opvec(H_f(X))^{\otimes 2} \right]\right) \geq \alpha.
	\end{align}
\end{assump}

In the remainder of this section we develop a number of bounds for $\norm{P_{L_{PCA}} - P_{\hat{L}}}_F$.
\begin{thm}\label{main_euc}
	Let $X_1, \dots, X_{m_x}$ be i.i.d random vectors in $\mathbb{R}^d$ such that they are bounded $\norm{X_i}_2 \leq 1$. 
	Denote by $P_{L_{PCA}}$, $P_{\hat{L}}$ the orthogonal projections onto the spaces spanned by the first $m+m_1$ left singular vectors of $M, \hat{M}$ (see (\ref{def_M}), (\ref{def_hatM})).
	If $\norm{\mathcal{O}^TX_i}_2^2$ is a sub-gaussian random variable such that $\mathbb{E}[\norm{\mathcal{O}^TX_i}_2^2]=\mu$, $\norm{\norm{\mathcal{O}^TX_i}_2^2 - \mu}_{\Psi_2} \leq K$  for any orthogonal matrix $\mathcal{O} \in \mathbb{R}^{d\times m}$ and
	\begin{align*}
	\sigma_{m+m_1}\left(\mathbb{E} \left[ \opvec(H_f(X_1))^{\otimes 2} \right]\right) \geq \alpha > 0,
	\end{align*}
	then we get
	\begin{align*}
	\norm{P_{L_{PCA}} - P_{\hat{L}}}_F \leq 2 C_1 \sqrt{\frac{(1+t)\mu}{\sqrt{(1-s)\alpha}}}
	\end{align*}
	for  $s \in (0,1), t > 0$, with probability at least  
	\begin{align*}
	1-2 \exp\left(- \frac{c t^2m_x \mu}{K^2}\right) -(m+m_1)\exp\left( \frac{-s^2 m_x \alpha}{C_2 m_1}\right),
	\end{align*} 
	and constants $C_1 = (1+\epsilon_A)^4 (1+2\epsilon_B) \eta_2 \left(\kappa_2^2  + 2\kappa_1\kappa_2 \right), C_2, c > 0$.
\end{thm}
The proof of Theorem \ref{MAIN} is an application of Wedin's bound (see Appendix Theorem \ref{wedin}), which bounds $\norm{P_{L_{PCA}} - P_{\hat{L}}}_F$ from above by the 
distance $\norm{M-\hat{M}}_F$ scaled by the spectral gap of $M$ and $\hat{M}$ at the $m+m_1$-th singular value. Before we give a proof, we introduce two auxiliary lemmas. 

\iffalse
\begin{lem}\label{boundnormsum}
	For $f\in \mathcal{F}_d(m_1,m)$ define
	\begin{align*}
	M = \left[ \opvec(H_f(\ve{x}_1))\middle| ...\middle| \opvec(H_f(\ve{x}_{m_x}))\right] \in \mathbb{R}^{d^2 \times m_x},\\
	\hat{M} = \left[  \opvec(P_L H_f(\ve{x}_1))\middle| ...\middle|  \opvec(P_L H_f(\ve{x}_{m_x}))\right] \in \mathbb{R}^{d^2 \times m_x},
	\end{align*}
	If $x_1, \dots, x_m \in \mathbb{R}^{d}$ such that $\norm{x_i}_2 \leq 1$ for all $i = 1,\dots, m_x$, then
	\begin{align*}
	\norm{M - \hat{M}}_F^2  \leq \tilde{C}_1^2 \sum^{m_x}_{i=1} \norm{A^T \ve{x}_i}^2_2,
	\end{align*}
	for $\tilde{C}_1 = (1+\epsilon_A)^3(1+2\epsilon_B)\eta_2(\kappa_2^2 + 2\kappa_1\kappa_2) >0$.
\end{lem}
\begin{proofrem}
	\color{red}
	Summary
	\begin{enumerate}
		\item Standalone, only inequalities
	\end{enumerate}
	\color{black}
\end{proofrem}
\begin{proof}[Proof of lemma \ref{boundnormsum}]
	First, note that
	\begin{align*}
	\norm{M-\hat{M}}_F^2 &= \sum_{i=1}^{m_x} \norm{\opvec(H_f(\ve{x}_i))- \opvec(P_L H_f(\ve{x}_i)) }^2_2. \\
	\end{align*}
	Now
	\begin{align}
	\begin{split}
	&\norm{\opvec(H_f(\ve{x}_i))- \opvec(P_L H_f(\ve{x}_i)) }_2 \\
	&= \norm{ \opvec( V_{\ve{x}_i} S_{\ve{x}_i} V^T_{\ve{x}_i}) + \opvec(A T_{\ve{x}_i} A^T ) -   \opvec(P_L V_{\ve{x}_i} S_{\ve{x}_i} V^T_{\ve{x}_i}) - \opvec(P_L A T_{\ve{x}_i} A^T )}_2\\
	&= \norm{\opvec( V_{\ve{x}_i} S_{\ve{x}_i} V^T_{\ve{x}_i})  - \opvec(P_L  V_{\ve{x}_i} S_{\ve{x}_i} V^T_{\ve{x}_i})}_2 = \norm{V_{\ve{x}_i} S_{\ve{x}_i} V^T_{\ve{x}_i}  - P_L V_{\ve{x}_i} S_{\ve{x}_i} V^T_{\ve{x}_i}}_F,
	\end{split}
	\end{align}
	where the last step is due to $A T_{\ve{x}_i} A^T  \in L$.
	Set $\Delta_{\ve{x}_i} = G_{\ve{x}_i} - G_0$ and denote $V := V_0= AG_0B$ then $\opvec(VS_{\ve{x}_i}V^T) \in L$. Since $P_L$ is an orthogonal projection, we continue with
	\begin{align*}
	&\norm{V_{\ve{x}_i} S_{\ve{x}_i} V^T_{\ve{x}_i}  - P_L V_{\ve{x}_i} S_{\ve{x}_i} V^T_{\ve{x}_i}}_F \\
	&\leq \norm{\opvec( V_{\ve{x}_i} S_{\ve{x}_i} V^T_{\ve{x}_i}) - \opvec(V S_{\ve{x}_i} V^T)}_F\\
	&= \norm{V_{\ve{x}_i} S_{\ve{x}_i} V^T_{\ve{x}_i} - V S_{\ve{x}_i} V^T}_F \\
	&= \norm{AG_{\ve{x}_i}B S_{\ve{x}_i} B^T G_{\ve{x}_i} A^T - AG_0B S_{\ve{x}_i} B^T G_0 A^T}_F\\
	&\leq(1+\epsilon_A)^2 \norm{G_{\ve{x}_i}B S_{\ve{x}_i} B^T G_{\ve{x}_i} - G_0 B S_{\ve{x}_i} B^TG_0}_F.\\
	&=(1+\epsilon_A)^2 \norm{(G_0+\Delta_{\ve{x}_i})B S_{\ve{x}_i} B^T (G_0 + \Delta_{\ve{x}_i}) - G_0 B S_{\ve{x}_i} B^T G_0}_F.\\
	&=(1+\epsilon_A)^2 \norm{\Delta_{\ve{x}_i}B S_{\ve{x}_i} B^T \Delta_{\ve{x}_i} + \Delta_{\ve{x}_i}B S_{\ve{x}_i} B^T G_0 + G_0 B S_{\ve{x}_i} B^T\Delta_{\ve{x}_i}}_F \\
	&\leq (1+\epsilon_A)^2 \left(\norm{\Delta_{\ve{x}_i}B S_{\ve{x}_i} B^T \Delta_{\ve{x}_i}}_F + 2 \norm{\Delta_{\ve{x}_i}B S_{\ve{x}_i} B^T G_0}_F\right)\\
	&\leq (1+\epsilon_A)^2 \left(\norm{\Delta_{\ve{x}_i}}^2_F\norm{B S_{\ve{x}_i} B^T} + 2 \norm{\Delta_{\ve{x}_i}}_F\norm{B S_{\ve{x}_i} B^T}\norm{G_0}\right)\\
	&\leq (1+\epsilon_A)^2(1+ 2\epsilon_B)  \norm{S_{\ve{x}_i}}\left(\norm{\Delta_{\ve{x}_i}}^2_F + 2\kappa_1\norm{\Delta_{\ve{x}_i}}_F\right).\\
	\end{align*}
	The elements of $S_{\ve{x}_i}$ are bounded by $\eta_2$, hence $\norm{S_{\ve{x}_i}} \leq \eta_2$ and $g_i'$ is Lipschitz continuous with Lipschitz constant $\kappa_2$ on $[-1,1]$ for all $i=1,\dots, m$, i.e. $\abs{g_i'(t) - g_i'(0)} \leq \kappa_2\abs{t}$ for all $t\in [-1,1]$. Hence
	\begin{align*}
	(1+\epsilon_A)^2(1+ 2\epsilon_B) \norm{S_{\ve{x}_i}}\left(\norm{\Delta_{\ve{x}_i}}^2_F + 2\kappa_1\norm{\Delta_{\ve{x}_i}}_F\right)\\
	\leq (1+\epsilon_A)^2(1+ 2\epsilon_B)\eta_2 \left(\kappa_2^2 \norm{A^T \ve{x}_i}^2_2 + 2 \kappa_1\kappa_2 \norm{A^T \ve{x}_i}_2\right) \\
	\leq (1+\epsilon_A)^3(1+ 2\epsilon_B) \eta_2 \left(\kappa_2^2  + 2\kappa_1\kappa_2 \right)\norm{A^T \ve{x}_i}_2,
	\end{align*}
	where we used $\norm{A^T \ve{x}_i}^2_2 \leq (1+\epsilon_A)\norm{A x_i}_2$ in the last step. By introducing the constant
	\begin{align}
	\tilde{C}_1 := (1+\epsilon_A)^3 (1+2\epsilon_B) \eta_2 \left(\kappa_2^2  + 2\kappa_1\kappa_2 \right) > 0,
	\end{align}
	we can now bound $\norm{M-\hat{M}}^2_F$ by
	\begin{align*}
	\norm{M-\hat{M}}^2_F \leq  \tilde{C}_1^2 \sum^{m_x}_{i=1} \norm{A^T \ve{x}_i}^2_2.
	\end{align*}
	
\end{proof}
\fi
\begin{lem}\label{boundnormconc}
	Let $X_1, \dots, X_{m_x}$ be i.i.d random vectors in $\mathbb{R}^d$, such that $\norm{X_i}_2 \leq 1$
	If $\norm{\mathcal{O}^TX_i}_2^2$ is sub-gaussian such that $\mathbb{E}[\norm{\mathcal{O}^TX_i}_2^2]=\mu$, $\norm{\norm{\mathcal{O}^TX_i}_2^2 - \mu}_{\Psi_2} \leq K$,  for any orthogonal matrix $\mathcal{O} \in \mathbb{R}^{d\times m}$, then
	\begin{align*}
	\norm{M-\hat{M}}_F \leq C_1\sqrt{(1+t)m_x \mu},
	\end{align*}        
	with probability at least $1 -  2 \exp\left(- \frac{c t^2m_x \mu}{K^2}\right)$ for some constant $c > 0$ and for all $t>0$, and $C_1 = (1+\epsilon_A)\tilde{C}_1 = (1+\epsilon_A)^4 (1+2\epsilon_B) \eta_2 \left(\kappa_2^2  + 2\kappa_1\kappa_2\right)$.
\end{lem}

\begin{proof}[Proof of Lemma \ref{boundnormconc}]
	Denote by $\bar{A}$ the optimal orthogonal matrix of $A$. Then by Lemma \ref{boundnormsum} 
		First, note that
	\begin{align*}
	\norm{M-\hat{M}}_F^2 &= \sum_{i=1}^{m_x} \norm{\opvec(H_f(\ve{x}_i))- \opvec(P_L H_f(\ve{x}_i)) }^2_2. \\
	\end{align*}
	Now
	\begin{align}
	\begin{split}
	&\norm{\opvec(H_f(\ve{x}_i))- \opvec(P_L H_f(\ve{x}_i)) }_2 \\
	&= \norm{ \opvec( V_{\ve{x}_i} S_{\ve{x}_i} V^T_{\ve{x}_i}) + \opvec(A T_{\ve{x}_i} A^T ) -   \opvec(P_L V_{\ve{x}_i} S_{\ve{x}_i} V^T_{\ve{x}_i}) - \opvec(P_L A T_{\ve{x}_i} A^T )}_2\\
	&= \norm{\opvec( V_{\ve{x}_i} S_{\ve{x}_i} V^T_{\ve{x}_i})  - \opvec(P_L  V_{\ve{x}_i} S_{\ve{x}_i} V^T_{\ve{x}_i})}_2 = \norm{V_{\ve{x}_i} S_{\ve{x}_i} V^T_{\ve{x}_i}  - P_L V_{\ve{x}_i} S_{\ve{x}_i} V^T_{\ve{x}_i}}_F,
	\end{split}
	\end{align}
	where the last step is due to $A T_{\ve{x}_i} A^T  \in L$.
	Set $\Delta_{\ve{x}_i} = G_{\ve{x}_i} - G_0$ and denote $V := V_0= AG_0B$ then $\opvec(VS_{\ve{x}_i}V^T) \in L$. Since $P_L$ is an orthogonal projection, we continue with
	\begin{align*}
	\norm{V_{\ve{x}_i} S_{\ve{x}_i} V^T_{\ve{x}_i}  - P_L V_{\ve{x}_i} S_{\ve{x}_i} V^T_{\ve{x}_i}}_F 
	&\leq \norm{\opvec( V_{\ve{x}_i} S_{\ve{x}_i} V^T_{\ve{x}_i}) - \opvec(V S_{\ve{x}_i} V^T)}_2\\
	&= \norm{V_{\ve{x}_i} S_{\ve{x}_i} V^T_{\ve{x}_i} - V S_{\ve{x}_i} V^T}_F \\
	&= \norm{AG_{\ve{x}_i}B S_{\ve{x}_i} B^T G_{\ve{x}_i} A^T - AG_0B S_{\ve{x}_i} B^T G_0 A^T}_F\\
	&\leq(1+\epsilon_A)^2 \norm{G_{\ve{x}_i}B S_{\ve{x}_i} B^T G_{\ve{x}_i} - G_0 B S_{\ve{x}_i} B^TG_0}_F.\\
	&=(1+\epsilon_A)^2 \norm{(G_0+\Delta_{\ve{x}_i})B S_{\ve{x}_i} B^T (G_0 + \Delta_{\ve{x}_i}) - G_0 B S_{\ve{x}_i} B^T G_0}_F.\\
	&=(1+\epsilon_A)^2 \norm{\Delta_{\ve{x}_i}B S_{\ve{x}_i} B^T \Delta_{\ve{x}_i} + \Delta_{\ve{x}_i}B S_{\ve{x}_i} B^T G_0 + G_0 B S_{\ve{x}_i} B^T\Delta_{\ve{x}_i}}_F \\
	&\leq (1+\epsilon_A)^2 \left(\norm{\Delta_{\ve{x}_i}B S_{\ve{x}_i} B^T \Delta_{\ve{x}_i}}_F + 2 \norm{\Delta_{\ve{x}_i}B S_{\ve{x}_i} B^T G_0}_F\right)\\
	&\leq (1+\epsilon_A)^2 \left(\norm{\Delta_{\ve{x}_i}}^2_F\norm{B S_{\ve{x}_i} B^T} + 2 \norm{\Delta_{\ve{x}_i}}_F\norm{B S_{\ve{x}_i} B^T}\norm{G_0}\right)\\
	&\leq (1+\epsilon_A)^2(1+ 2\epsilon_B)  \norm{S_{\ve{x}_i}}\left(\norm{\Delta_{\ve{x}_i}}^2_F + 2\kappa_1\norm{\Delta_{\ve{x}_i}}_F\right).
	\end{align*}
	The elements of $S_{\ve{x}_i}$ are bounded by $\eta_2$, hence $\norm{S_{\ve{x}_i}} \leq \eta_2$ and $g_i'$ is Lipschitz continuous with Lipschitz constant $\kappa_2$ on $[-1,1]$ for all $i=1,\dots, m$, i.e. $\abs{g_i'(t) - g_i'(0)} \leq \kappa_2\abs{t}$ for all $t\in [-1,1]$. Hence
	\begin{align*}
	(1+\epsilon_A)^2(1+ 2\epsilon_B) \norm{S_{\ve{x}_i}}\left(\norm{\Delta_{\ve{x}_i}}^2_F + 2\kappa_1\norm{\Delta_{\ve{x}_i}}_F\right)\\
	\leq (1+\epsilon_A)^2(1+ 2\epsilon_B)\eta_2 \left(\kappa_2^2 \norm{A^T \ve{x}_i}^2_2 + 2 \kappa_1\kappa_2 \norm{A^T \ve{x}_i}_2\right) \\
	\leq (1+\epsilon_A)^3(1+ 2\epsilon_B) \eta_2 \left(\kappa_2^2  + 2\kappa_1\kappa_2 \right)\norm{A^T \ve{x}_i}_2,
	\end{align*}
	where we used $\norm{A^T \ve{x}_i}^2_2 \leq (1+\epsilon_A)\norm{A x_i}_2$ in the last step. By introducing the constant
	\begin{align}
	\tilde{C}_1 := (1+\epsilon_A)^3 (1+2\epsilon_B) \eta_2 \left(\kappa_2^2  + 2\kappa_1\kappa_2 \right) > 0,
	\end{align}
	we can now bound $\norm{M-\hat{M}}^2_F$ by
	\begin{align*}
	\norm{M-\hat{M}}^2_F \leq  \tilde{C}_1^2 \sum^{m_x}_{i=1} \norm{A^T \ve{x}_i}^2_2.
	\end{align*}
	Here missing link:
	\begin{align}
	\norm{M - \hat{M}}_F^2  \leq \tilde{C}_1^2 m_1 \sum^{m_x}_{i=1} \norm{A^T \ve{x}_i}^2_{\infty}.
	\end{align}
	\color{black}
	
	\begin{align*}
	&\norm{M-\hat{M}}^2_F \leq \tilde{C}_1^2 \sum^{m_x}_{i=1} \norm{A^T \ve{X}_i}^2_2 \\ \leq& (1+\epsilon_A)^2 \tilde{C}_1^2 \sum^{m_x}_{i=1} \norm{\bar{A}^T \ve{X}_i}^2_2
	=  C_1^2 \sum^{m_x}_{i=1} \norm{\bar{A}^T \ve{X}_i}^2_2
	\end{align*}
	for $C_1 = (1+\epsilon_A)\tilde{C}_1$.
	Set $Y_i := \norm{\bar{A}^T X_i}^2_2$. Then by our assumption $\mathbb{E}[Y_i] = \mu$ and  $\norm{Y_i - \mu}_{\Psi_2} \leq K$. Therefore we get
	\begin{align*}
	\mathbb{P}\left[\sum^{m_x}_{i=1} \norm{\bar{A}^T \ve{X}_i}^2_2 \geq (1+t) m_x \mu \right] \leq \mathbb{P}\left[\sum^{m_x}_{i=1} \abs{Y_i - \mathbb{E}[Y_i]} \geq t m_x \mu \right].
	\end{align*}
	By Hoeffding's concentration inequality for sub-gaussian random variables (Appendix Theorem \ref{hoeffdingsubgaussian}), we get for some constant $c>0$ and $t > 0$
	\begin{align*}
	\mathbb{P}\left[\sum^{m_x}_{i=1} \abs{Y_i - \mathbb{E}[Y_i]} \geq t m_x \mu \right] \leq 2 \exp\left(- \frac{ct^2 m_x^2 \mu^2}{\sum^{m_x}_{i=1}\norm{Y_i - \mathbb{E}[Y_i]}^2_{\psi_2}}\right)\\
	\leq  2 \exp\left(- \frac{c t^2m_x \mu^2 }{K^2}\right).
	\end{align*}
	Thus
	\begin{align*}
	\norm{M-\hat{M}}_F \leq C_1\sqrt{(1+t)m_x \mu },
	\end{align*}
	with probability at least
	\begin{align*}
	1 -  2 \exp\left(- \frac{c t^2m_x \mu^2}{K^2}\right).
	\end{align*}
\end{proof}
\begin{lem}\label{boundsv}
	Let $X_1, \dots, X_{m_x}$ be i.i.d. random vectors, such that $\norm{ X_i}_2 \leq 1$. For $f \in \mathcal{F}_d(m_1, m)$ denote 
	\begin{align*}
	M = \left[ \opvec(H_f(\ve{X}_1))\middle| ...\middle| \opvec(H_f(\ve{X}_{m_x}))\right] \in \mathbb{R}^{d^2 \times m_x}.
	\end{align*}
	Assume that
	\begin{align*}
	\sigma_{m+m_1}(\mathbb{E}[ \opvec(H_f(\ve{X}_1))^{\otimes 2}]) \geq \alpha > 0.
	\end{align*}
	Then the $m+m_1$-th singular value of $M$ is bounded by
	\begin{align*}
	\sigma_{m+m_1}(M) \geq \sqrt{(1-t)m_x\alpha},
	\end{align*}
	with probability at least 
	\begin{align*}
	1-  (m+m_1)e^{-t^2 \frac{m_x \alpha}{C_2 m_1}}
	\end{align*}
	for any $0<t\leq 1$ and $C_2 = 2(1+\epsilon_A)^4(1+2\epsilon_B)^2 (\kappa_1^2 \eta_2 + \kappa_2\eta_1)^2$.
\end{lem}



\begin{proof}[Proof of Lemma \ref{boundsv}]
	%Setting the color to red to indacte that this part is unfinished
	Let $\ve{x} \in \mathbb{R}^d, \norm{x}_2 \leq 1$, then 
	\begin{align*}
	\norm{\opvec(H_f(\ve{x}))}_2 &= \norm{H_f(\ve{x})}_F \\
	&=\norm{\ma{A}\ma{G}_{\ve{x}}\ma{B}\ma{S}_{\ve{x}}\ma{B}^T \ma{G}_{\ve{x}} \ma{A}^T + \ma{A} \ma{T}_x \ma{A}^T }_F\\
	&\leq (1+\epsilon_A)^2\norm{\ma{G}_{\ve{x}}\ma{B}\ma{S}_{\ve{x}}\ma{B}^T \ma{G}_{\ve{x}}}_F  + (1+2\epsilon_A)\norm{\ma{T}_x }_F.
	\end{align*}
	We start with a bound for $\norm{\ma{T}_x }_F$. Recall that we defined $S_x \in \mathbb{R}^{m_1 \times m_1}, \ma{T}_x \in \mathbb{R}^{m\times m}$ in (\ref{def_S} - \ref{def_T}). The diagonal elements of $T_x$ were given as  $\ma{T}_{\ve{x}, ii} = \left[\ma{B}^T h'(\ma{B}^T g(\ma{A}^T \ve{x})) \right]_i g_i''(\ve{a}_i^T \ve{x})$. Let $\ve{t}_x$ be the vector built from the diagonal elements of $\ma{T}_x$ and denote by "$\cdot$" the elementwise vector multiplication. Then $\norm{\ma{T}_x}_F = \norm{\ve{t}_x}_2 $ and 
	\begin{align*}
	\norm{\ve{t}_x}_2 &= \norm{\ma{B}h'(\ma{B}^T g(\ma{A}^T \ve{x})) \cdot g''(\ma{A}^T \ve{x})}_2 \leq \kappa_2 \norm{\ma{B}h'(\ma{B}^T g(\ma{A}^T \ve{x}))}_2\\
	&\leq \kappa_2 \norm{\ma{B}} \norm{h'(\ma{B}^T g(\ma{A}^T \ve{x}))}_2 \leq (1+\epsilon_B)\kappa_2 \norm{h'(\ma{B}^T g(\ma{A}^T \ve{x}))}_2\\
	&= (1+\epsilon_B) \kappa_2 \left(\sum_{\ell=1}^{m_1} h_\ell'(\ve{b}_\ell^T g(\ma{A}^T \ve{x}))^2\right)^{\frac{1}{2}} \leq (1+\epsilon_B)\kappa_2 \eta_1 \sqrt{m_1}.
	\end{align*}
	The other norm can be estimated by
	\begin{align*}
	\norm{\ma{G}_{\ve{x}}\ma{B}\ma{S}_{\ve{x}}\ma{B}^T \ma{G}_{\ve{x}}}_F &\leq \norm{G_x}^2 \norm{\ma{B}\ma{S}_x \ma{B}^T}_F\\
	&\leq (1+2\epsilon_B) \kappa_1^2 \norm{\ma{S}_x}_F \leq (1+2\epsilon_B) \kappa_1^2 \eta_2 \sqrt{m_1}.
	\end{align*}
	Thus $\norm{\opvec(H_f(\ve{x}))}_2 \leq (1+\epsilon_A)^2(1+2\epsilon_B)(\kappa_1^2\eta_2 + \kappa_2\eta_1)\sqrt{m_1}$.  Note that 
	\begin{align}
	\sigma_{m+m_1}(\ma{M}) &= \sqrt{\sigma_{m+m_1}(\ma{M}\ma{M}^T)} = \sqrt{\sigma_{m+m_1}\left(\sum_{i=1}^{m_x} \opvec(H_f(\ve{x}_i))^{\otimes 2}\right)}.\label{switch_representation}
	\end{align}
	The sum $\sum_{i=1}^{m_x} \opvec(H_f(\ve{X}_i))^{\otimes 2}$ consists of independent random matrices. The summands $\opvec(H_f(\ve{X}_i))^{\otimes 2}$ are clearly positive semidefinite: 
	\begin{align*}
	\ve{z}^T \opvec(H_f(\ve{X_i}))^{\otimes 2} \ve{z} = \left(\opvec(H_f(\ve{X_i}))^T \ve{z}\right)^2  \geq 0 \text{ for all } \ve{z} \in \mathbb{R}^{d^2}.
	\end{align*}
	This allows us to use the Chernoff concentration inequality for the inner singular values developed by  Gittens and Tropp \cite{tropp_inner}, see Appendix Theorem \ref{tropp_inner}. We will see that the conditions of the theorem trivialize in our case. Let
	\begin{align*}
	\mathbb{E}[\opvec(H_f(\ve{X}))^{\otimes 2}] = \ma{W}\ma{\Lambda}\ma{W^T}
	\end{align*}  
	be the spectral decomposition of $\mathbb{E}[\opvec(H_f(\ve{X}))^{\otimes 2}]$. Denote by $\ve{w}_i$ the $i$-th eigenvector. Since $\opvec(H_f(\ve{X}))^{\otimes 2}$ is positive semidefinite, the same is true for its expectation, so all eigenvalues are non-negative. Further, we can assume the eigenvalues are ordered by their magnitude:
	\begin{align*}
	\ma{\Lambda}_1 \geq ... \geq \ma{\Lambda}_{d^2} \geq 0.
	\end{align*}
	Note that this implies $\ma{\Lambda}_{m+m_1} = \sigma_{m+m_1}(\mathbb{E}[\opvec(H_f(\ve{X}))^{\otimes 2}]) \geq \alpha$, we can assume that $\alpha$ is such that we have equality $\ma{\Lambda}_{m+m_1}=\alpha$. Now, set
	\begin{align*}
	\ma{W}_- = (\ve{w}_1| \ve{w}_2 | \dots |\ve{w}_{m+m_1}) \in \mathbb{R}^{d^2 \times m+m_1}\, \text{ and } \, \ma{W}_+ = (\ve{w}_{m+m_1}| \dots |\ve{w}_{d^2}) \in \mathbb{R}^{d^2 \times (d^2 - m - m_1 +1)}.
	\end{align*}
	Since all $ \opvec(H_f(\ve{X}_i))^{\otimes 2}$ are i.i.d and therefore share the same mean  we have
	\begin{align*}
	\mu_{m+m_1} = \lambda_{max}\left( \sum_{j=1}^{m_x}\ma{W}_+^T(\mathbb{E}[\opvec(H_f(\ve{X}_i))^{\otimes 2}])\ma{W}_+ \right) = m_x\alpha,
	\end{align*}
	and
	\begin{align*}
	\mu_{m+m_1} = \lambda_{min}\left( \sum_{j=1}^{m_x}\ma{W}_-^T(\mathbb{E}[\opvec(H_f(\ve{X}_i))^{\otimes 2}])\ma{W}_- \right) = m_x\alpha.
	\end{align*}
	We established that $\norm{\opvec(H_f(\ve{X}))}_2$ is bounded, therefore we can set 
	\begin{align*}
	\Psi(\ma{W}) &= \norm{\opvec(H_f(\ve{X}))^{\otimes 2}} \leq \norm{\opvec(H_f(\ve{X}))^{\otimes 2}}_F \\
	&\leq  \norm{\opvec(H_f(\ve{X}))}_2^2 \leq  \frac{1}{2}C_2 m_1,
	\end{align*}
	with $C_2 := 2(1+\epsilon_A)^4(1+2\epsilon_B)^2(\kappa^2_1 \eta_2 + \kappa_2 \eta_1)^2$.
	
	By Theorem \ref{tropp_inner} (Appendix)  
	\begin{align*}
	\mathbb{P} \left[ \lambda_{m+m_1}\left(\sum_{i=1}^{m_x} \opvec(H_f(\ve{X_i}))^{\otimes 2} \right) \leq (1-t)m_x \alpha \right] \leq (m+m_1)e^{-t^2 \frac{m_x \alpha}{C_2 m_1}}.
	\end{align*}
	We used the eigenvalues to stay consistent with the notation from the theorem, but since all involved matrices were symmetric and positive semidefinite, the same statement is true for the $m+m_1$-th singular value of $\sum_{i=1}^{m_x} \opvec(H_f(\ve{X_i}))^{\otimes 2}$. Therefore, and by (\ref{switch_representation}), we have
	\begin{align*}
	\sigma_{m+m_1}(M) \geq \sqrt{(1-t)m_x\alpha}
	\end{align*}
	with probability at least $1-(m+m_1)e^{-t^2 \frac{m_x \alpha}{C_2 m_1}}$ for any $0<t\leq 1$.
\end{proof}
\begin{proof}[Proof of Theorem \ref{MAIN}]
	The proof is an application of the previous lemmas together with Wedin's bound. Given $M,\hat{M}$ let 
	\begin{align*}
	\ma{M} &= \begin{pmatrix}\ma{U}_1 & \ma{U}_2\end{pmatrix}
	\begin{pmatrix}\ma{\Sigma}_1 &0 & 0 \\ 0 &  \ma{\Sigma}_2 & 0\end{pmatrix}
	\begin{pmatrix}\ma{V}^T_1 \\ \ma{V}^T_2\end{pmatrix},\\
	\ma{\hat{M}} &= \begin{pmatrix}\ma{\hat{U}}_1 & \ma{\hat{U}}_2\end{pmatrix}
	\begin{pmatrix}\ma{\hat{\Sigma}}_1 &0 & 0\\ 0 & \ma{\hat{\Sigma}}_2 & 0\end{pmatrix}
	\begin{pmatrix}\ma{\hat{V}}^T_1 \\ \ma{\hat{V}}^T_2\end{pmatrix},
	\end{align*}
	be the singular value decomposition of $\ma{M},\hat{\ma{M}}$, where $\ma{\Sigma}_1, \ma{\hat{\Sigma}}_1 \in \mathbb{R}^{m+m_1 \times m+m_1}$ and so on. Note that since $L$ has dimension $m+m_1$ and $\ma{\hat{M}}$ is the projection of the columns onto $L$, the rank of $\hat{\ma{M}}$ can not be greater than $m+m_1$. Therefore $\ma{\hat{\Sigma}}_2 = 0$. Denote by $P_{L_{PCA}}$, $P_{\hat{L}}$ the projections onto the spaces spanned by the first $m+m_1$ left singular vectors of $M, \hat{M}$. By Wedin's bound (Appendix Theorem \ref{wedin}), we have 
	\begin{align*}
	\norm{P_{L_{PCA}} - P_{\hat{L}}}_F \leq \frac{2 \norm{\ma{M} - \ma{\hat{M}}}_F}{\bar{\alpha}},
	\end{align*}
	where $\bar{\alpha} \geq \min_{k, \hat{k}} \abs{ \sigma_{\hat{k}} (\hat{\ma{\Sigma}}_2) - \sigma_k(\ma{\Sigma}_1) }$ and $\bar{\alpha} \geq  \min_{k} \abs{ \sigma_{k}(\ma{\Sigma}_1)}$.
	Since $\norm{X_i}_2 \leq 1$ and $\mathbb{E} \left[ \opvec(H_f(X_1))^{\otimes 2} \right] \geq \alpha$, Lemma \ref{boundsv} yields
	\begin{align*} 
	\sigma_{m+m_1}(M) \geq \sqrt{(1-s)m_x\alpha}
	\end{align*}
	with probability at least $1-  (m+m_1)e^{-s^2 \frac{m_x \alpha}{C_2 m_1}}$. 
	This, together with the fact that $\ma{\hat{\Sigma}}_2 = 0$, allows us to set $\bar{\alpha} = \sqrt{(1-s)m_x\alpha}$. 
	By Lemma \ref{boundnorm}, we have 
	\begin{align*}
	\norm{M-\hat{M}}_F \leq C_1\sqrt{(1+t)m_x \mu},
	\end{align*}        
	with probability at least $1 -  2 \exp\left(- \frac{c t^2m_x \mu}{K^2}\right)$. Combining these with the union bound for probabilities yields
	\begin{align*}
	\norm{P_{L_{PCA}} - P_{\hat{L}}}_F \leq 2\frac{C_1\sqrt{(1+t)m_x \mu}}{\sqrt{(1-s)m_x\alpha}} = 2 C_1 \sqrt{\frac{(1+t)\mu}{\sqrt{(1-s)\alpha}}},
	\end{align*}
	with probability at least  
	\begin{align*}
	1-2 \exp\left(- \frac{c t^2m_x \mu}{K^2}\right) -(m+m_1)\exp\left( \frac{-s^2 m_x \alpha}{C_2 m_1}\right), 
	\end{align*} 
	for $s \in (0,1), t > 0$. The constants $C_1,C_2, c >0$ are taken from the respective lemmas.
\end{proof}

\iffalse

Note the immediate consequence of Theorem \ref{MAIN} on Algorithm 1 is:

\begin{cor}\label{MAINWEDIN}
	Under Assumption \ref{assump:lowersvbound} (cf. (\ref{alpha_bound})) Algorithm \ref{alg:dimred} applied to a function $f \in \mathcal{F}_d(m_1,m)$ produces $L_{PCA}$ such that 
	\begin{align}
	\norm{P_{L_{PCA}} - P_{\hat{L}}}_F \leq 2C_1 \sqrt{\frac{(1+t) m}{(1-s) \alpha d}}
	\end{align}
	with constant $C_1 = (1+\epsilon_A)^4 (1+2\epsilon_B) \eta_2 \left(\kappa_2^2  + 2\kappa_1\kappa_2 \right)$ and probability at least  
	\begin{align*}
	1-2  \exp\left( -\frac{C_3 t^2m_x m^2}{d}\right) -(m+m_1)\exp\left( \frac{-s^2 m_x \alpha}{C_2 m_1}\right), 
	\end{align*} 
	for $C_2, C_3 > 0$ constant and $0 < s <1, t > 0.$
\end{cor}

\begin{proof}
	Follows directly from Theorem \ref{MAIN} together with Corollary \ref{bound_norm_cor}.
\end{proof}

\fi


The results above guarantee some bound on $\norm{{P_{L_{PCA}}}-P_{\hat{L}}}_F$. What remains is to show that $L^{vec}$ and $\hat{L}$ are close. 
\begin{prop}
	Let $f \in \mathcal{F}_d(m_1,m)$ and denote by $L^{vec}, \hat{L}, L_{PCA}$ the spaces defined above.
	If $\norm{{P_{L_{PCA}}}-P_{\hat{L}}}_F \leq \epsilon$ for $0 \leq \epsilon < 1$,  then $\hat{L}$ and $L^{vec}$ span the same space.
\end{prop}
\begin{proof}
	Assume $\norm{{P_{L_{PCA}}}-P_{\hat{L}}}_F \leq \epsilon$ for $0 \leq \epsilon < 1$. The space $\hat{L}$ is constructed by the columns of $\ma{\hat{M}}$ which lie in $L^{vec}$, therefore $\hat{L}$ has to be a subspace of $L^{vec}$. By {Theorem \ref{thm:independenceL}} we know that $L$ is spanned by $m+m_1$ independent elements. Therefore 
	\begin{align*}
	\operatorname{dim}(L^{vec}) = \operatorname{dim}(L)= m+m_1,
	\end{align*}
	and we have $\hat{L} = L^{vec}$ if $\operatorname{dim}(\hat{L}) = m+m_1$. Assume that $\operatorname{dim}(\hat{L}) < m+m_1$. Since $\operatorname{dim}(L_{PCA}) = m+m_1$, we can find an element $\ve{x} \in L_{PCA}$ that is orthogonal to $\hat{L}$, w.l.o.g $\norm{x}_2=1$. Now consider the distance of the projections of $x$:
	\begin{align*}
	\norm{P_{L_{PCA}}x - P_{\hat{L}}x}_2 \leq \norm{P_{L_{PCA}} - P_{\hat{L}}}_F \norm{x}_2 \leq \epsilon. 
	\end{align*}
	However, since $x$ lies in $L_{PCA}$ and is orthogonal to $P_{\hat{L}}$:
	\begin{align*}
	\norm{P_{L_{PCA}}x - P_{\hat{L}}x}_2 = \norm{x - 0}_2 = 1.
	\end{align*}
	Thus, $\operatorname{dim}(\hat{L})$ can not be smaller than $m+m_1$.
\end{proof}
To some extent, Theorem \ref{MAINWEDIN} already implies that $L^{vec} = \hat{L}$. If $f\in \mathcal{F}_d(m_1,m)$ is such that Theorem \ref{MAINWEDIN} yields $\norm{L_{PCA} - \hat{L}}_F < 1$, then  $L^{vec} = \hat{L}$ with the same probability. \\\\
The following proposition is a slight variation of Corollary \ref{MAINWEDIN}. It might provide a better bound, especially if $m_1$ is much smaller than $m$.
\begin{thm}\label{MAINLOG}
	Under Assumption \ref{assump:lowersvbound} (cf.(\ref{alpha_bound})) Algorithm \ref{alg:dimred} produces $L_{PCA}$ such that 
	\begin{align}
	\norm{P_{L_{PCA}} - P_{\hat{L}}}_F \leq 2C_1 \sqrt{\frac{(1+t) m_1}{(1-s) \alpha } \left(\sqrt{\frac{2\log(m)}{d}} + \frac{1}{d}\right)}
	\end{align}
	for $C_1 = (1+\epsilon_A)^4 (1+2\epsilon_B) \eta_2 \left(\kappa_2^2  + 2\kappa_1\kappa_2 \right)$, and with probability at least  
	\begin{align*}
	1- 2\exp(-2C_3t^2  m_x d^{-1}) -(m+m_1)\exp\left( \frac{-s^2 m_x \alpha}{C_2 m_1}\right)
	\end{align*} 
	for $C_2, C_3 > 0$ constant and $s \in (0,1), t > 0.$
\end{thm}

\begin{proof}
	The proof is very similar to the previous ones, so we will only point out the modifications and use the theory above where possible. Using the notation from the proof of Lemma \ref{boundnorm2} we had
	\begin{align*}
	\norm{M - \hat{M}}_F^2 \leq \sum^{m_x}_{i=1}  \norm{\opvec(H_f(x_i)) -  \opvec(P_L H_f(x_i))}_2^2, 
	\end{align*}
	together with a upper bound for the columns given by
	\begin{align*}
	\norm{\opvec(H_f(x_i)) - \opvec(P_L  H_f(x_i))}_2 \\\leq (1+\epsilon_A)^2 \left(\norm{\Delta_{\ve{x}_i}B S_{\ve{x}_i} B^T \Delta_{\ve{x}_i}}_F + 2 \norm{\Delta_{\ve{x}_i}B S_{\ve{x}_i} B^T G_0}_F\right)
	\end{align*}
	for $\Delta_{\ve{x}_i} = G_{x_i} - G_0$. By slightly changing the next steps in the proof of Lemma \ref{boundnorm2}, we get
	\begin{align*}
	&(1+\epsilon_A)^2 \left(\norm{\Delta_{\ve{x}_i}B S_{\ve{x}_i} B^T \Delta_{\ve{x}_i}}_F + 2 \norm{\Delta_{\ve{x}_i}B S_{\ve{x}_i} B^T G_0}_F\right)\\
	&\leq (1+\epsilon_A)^2 \left(\norm{\Delta_{\ve{x}_i}}^2 \norm{B S_{\ve{x}_i} B^T}_F + 2 \norm{\Delta_{\ve{x}_i}}\norm{G_0}\norm{B S_{\ve{x}_i} B^T}_F\right)\\
	&\leq (1+\epsilon_A)^2(1+2\epsilon_B)\left(\norm{\Delta_{\ve{x}_i}}^2 \norm{S_{\ve{x}_i}}_F + 2 \norm{\Delta_{\ve{x}_i}}\norm{G_0}\norm{S_{\ve{x}_i}}_F\right)\\
	&\leq (1+\epsilon_A)^2(1+2\epsilon_B)\eta_2 \sqrt{m_1} \left(\norm{\Delta_{\ve{x}_i}}^2  + 2 \kappa_1 \norm{\Delta_{\ve{x}_i}}\right).\\
	\end{align*}
	Instead of $\norm{\Delta_{\ve{x}_i}}_F$ we now have $\sqrt{m_1} \norm{\Delta_{\ve{x}_i}}$. Since $\Delta_{\ve{x}_i}$ is diagonal, it reduces to
	\begin{align*}
	\norm{\Delta_{\ve{x}_i}} = \norm{g'(A^T x_i) - g'(0)}_{\infty} \leq \kappa_2 \norm{A^T x_i}_{\infty},
	\end{align*}
	where $\norm{.}_{\infty}$ denotes the maximum norm for vectors. Therefore, one gets a slightly modified version of Lemma \ref{boundnorm2}:
	\begin{align}\label{newboundnorm}
	\norm{M - \hat{M}}_F^2  \leq \tilde{C}_1^2 m_1 \sum^{m_x}_{i=1} \norm{A^T \ve{x}_i}^2_{\infty}.
	\end{align}
	Let $\bar{A}$ be the optimal orthogonal matrix w.r.t. $A$ and denote $Y_i = \norm{\bar{A}^T \ve{X}_i}^2_{\infty}$, where $X_1, \dots X_{m_x} \sim \Unif(\mathbb{S}^{d-1})$ independently. Denote $\mu = \mathbb{E}[Y_i]$. Then, by Lemma \ref{meansupnorm},
	\begin{align*}
	\mu \leq \sqrt{\frac{2\log{m}}{d}} + \frac{1}{d},
	\end{align*}
	as well as $\norm{Y_i - \mathbb{E}[Y_i]}^2_{\Psi_2} \leq \frac{C}{2d+4}$ for some constant $C>0$ according to the results in the previous section. Additionally, we have 
	\begin{align*}
	\mu \geq \frac{1}{d},
	\end{align*}
	simply because the squared first coordinate of a vector that is drawn uniformly from the unit sphere has mean equal to $1/d$. Applying the arguments in the proof of Lemma \ref{boundnorm} to (\ref{newboundnorm}) results in 
	\begin{align*}
	\norm{M - \hat{M}}_F \leq C_1 \sqrt{(1+t)m_1 m_x \mu},
	\end{align*}
	with probability at least $1 - 2 \exp(-2ct^2  m_x d\mu^2)$, for some positive constant $c>0$. Using the bounds for both sides of $\mu$ gives
	
	\begin{align}\label{newboundnorm2}
	\norm{M - \hat{M}}_F \leq C_1 \sqrt{(1+t)m_1 m_x \left( \sqrt{\frac{2\log{m}}{d}} + \frac{1}{d}\right)},
	\end{align}
	with probability at least $1 - 2 \exp(-2ct^2  m_x d^{-1}) $ since, by $\mu \geq \frac{1}{d}$, 
	\begin{align*}
	1 - 2 \exp(-2ct^2  m_x d^{-1}) \leq 1 - 2 \exp(-2ct^2  m_x d\mu^2).
	\end{align*}
	The following steps are equivalent to the proof of Theorem \ref{MAIN}: we use Lemma \ref{boundsv} to receive a bound on the $m+m_1$-th singular value, then apply Wedin's bound with (\ref{newboundnorm2}) in the numerator. This yields
	\begin{align*}
	\norm{P_{L_{PCA}} - P_{\hat{L}}}_F \leq 2C_1 \sqrt{\frac{(1+t) m_1}{(1-s) \alpha } \left(\sqrt{\frac{2\log(m)}{d}} + \frac{1}{d}\right)},
	\end{align*}
	with probability at least
	\begin{align*}
	1 - 2 \exp(-2ct^2  m_x d^{-1}) - (m+m_1)\exp\left( \frac{-s^2 m_x \alpha}{C_2 m_1}\right).
	\end{align*}
	Setting $C_3 := c$ finishes the proof.
\end{proof}


==> sections/matrix_subspace/subsection3_finitedifferences.tex <==
\subsection{Approximation of the Hessians}
At the beginning of the last section we already pointed out that the Hessians $H[f](\ve{x})$ are in general not available. Therefore, we have to factor in the error caused by approximating $H[f](\ve{x})$. The approximation is done by finite differences. 
Denote by $e_i$ the $i$-th euclidean standard vector in $\mathbb{R}^d$. The approximation of the gradients $\nabla f(x)$ via finite differences is denoted by $\Delta_{\epsilon}[f](x)$, where $\epsilon > 0$ is usually very small and 
\begin{align*}
\Delta_\epsilon[f](\ve{x})_{i} := \frac{f(\ve{x} + \epsilon \ve{e}_i) - f(\ve{x})}{\epsilon} \text{ for } i=1,..., d.
\end{align*}
Similarly, we denote by $\Delta_\epsilon^2[f](\ve{x})$ the approximation of $H[f](x)$, which is given by
\begin{align*}
\Delta_{\epsilon}^2[f](\ve{x})_{ij} := \frac{f(\ve{x} + \epsilon \ve{e}_i + \epsilon \ve{e}_j) - f(\ve{x} + \epsilon \ve{e}_i) - f(\ve{x} + \epsilon \ve{e}_j) + f(\ve{x})}{\epsilon^2}
\end{align*}
for $i,j = 1,\dots, d$. In both scenarios we will refer to $\epsilon>0$ as the step size of the approximation. 
The following lemmas give an upper bound for the approximation error for our type of function.\\
To make the following estimates more understandable, we restate the setting of this chapter. As before, we only consider functions $f \in \mathcal{F}_d(m_1,m)$ that fulfill the properties of Definition \ref{def:f}. We refer to $A, B$ as the matrices with columns $a_1, \dots, a_m$, $b_1, \dots, b_{m_1}$, which are taken directly from the representation given in Definition \ref{def:f}. This also implies that $\norm{a_i}_2,\norm{b_\ell}_2 \leq 1$. Instead of referencing the elements of these vectors directly, we write them as elements of the matrices $A,B$. For example: $a_{ki}$ is the $k^{th}$ coordinate of the vector $a_i$ (for $i\leq m$).
The constants $\kappa_i, \eta_j$ are the ones that were defined in (\ref{kappa}) and (\ref{eta}). 
\begin{lem}\label{errorgrad}
	Let $\epsilon > 0$ and $\norm{x}_2 \leq 1$. Set $C_4 = 2 \max\set{\kappa_1^2 \eta_2,\kappa_2 \eta_1} > 0$,  then 
	\begin{align}
	\norm{\nabla f(x) - \Delta_{\epsilon}[f](x)}_2 \leq C_4 \epsilon  m_1 m.
	\end{align}
\end{lem}
\begin{proof}
	For fixed $k \in \set{1,...,d}$ we define $\phi(t) = f(x + te_k) - f(x)$. By the mean value theorem there exists a $0 < \xi_{k} < \epsilon$ such that
	\begin{align*}
	\Delta_{\epsilon}[f](x)_k &= \frac{\phi(\epsilon) - \phi(0)}{\epsilon} = \phi'(\xi_{k}) \\
	&= \nabla f(x + \xi_k e_k)^T e_k \\
	&= \frac{\partial f}{\partial x_k}(x + \xi_k e_k).
	\end{align*}
	Recall that by (\ref{gradient}) the partial derivatives of $f$ are 
	\begin{align*}
	\frac{\partial f}{\partial x_k}(x) = \sum^{m_1}_{\ell=1}\sum^m_{i=1}b_{i\ell}h_\ell'(b_\ell^Tg(A^T x)) g_i'(a_i^T x)a_{ki}.
	\end{align*}
	Fix $k$ for now and set $\tilde{x} = x + \xi_k e_k$. Then 
	\begin{align*}
	\left|\nabla f(x)_k - \Delta_{\epsilon}[f](x)_k \right| &= \left|\frac{\partial f}{\partial x_k}(x) - \frac{\partial f}{\partial x_k}(\tilde{x})\right| \\
	&= \left| \sum^{m_1}_{\ell=1}\sum^m_{i=1}b_{i\ell}\left[h_\ell'(b_\ell^Tg(A^T x)) g_i'(a_i^T x) - h_\ell'(b_\ell^Tg(A^T \tilde{x})) g_i'(a_i^T \tilde{x})\right]a_{ki} \right| .
	\end{align*} 
	For the inner part of the sum we get
	\begin{align*}
	&\abs{h_\ell'(b_\ell^T g(A^T x))g_i'(a_i^T x) - h_\ell'(b_\ell^T g(A^T \tilde{x}))g_i'(a_i^T \tilde{x})} \\
	\leq& \abs{h_\ell'(b_\ell^T g(A^T x))g_i'(a_i^T x) - h_\ell'(b_\ell^T g(A^T x))g_i'(a_i^T \tilde{x})} \\
	+& \abs{h_\ell'(b_\ell^T g(A^T x))g_i'(a_i^T \tilde{x}) - h_\ell'(b_\ell^T g(A^T \tilde{x}))g_i'(a_i^T \tilde{x})} \\
	\leq& \eta_1 \abs{g_i'(a_i^T x) - g_i'(a_i^T \tilde{x})} + \kappa_1 \abs{h_\ell'(b_\ell^T g(A^T x)) - h_\ell'(b_\ell^T g(A^T \tilde{x}))}\\
	\leq& \eta_1 \kappa_2 \abs{a_i^T(x - \tilde{x})} + \kappa_1 \eta_2 \abs{ b_\ell^T(g(A^T x) - g(A^T \tilde{x})) } \\
	\leq& \eta_1 \kappa_2 \abs{a_{ki}\xi_k} + \kappa_1^2 \eta_2  \sum^m_{j=1} \abs{b_{j\ell}a_{kj}\xi_k }\\
	\leq& \eta_1 \kappa_2 \epsilon \abs{a_{ki}} + \kappa_1^2 \eta_2 \epsilon\abs{ \sum^m_{j=1} b_{j\ell}a_{kj}}.
	\end{align*}
	Hence, with  $\tilde{C}_4 := \max \set{\eta_1 \kappa_2, \kappa_1^2 \eta_2}$, we get 
	\begin{align*}
	&\left\vert \frac{\partial f}{\partial x_k}(x) - \frac{\partial f}{\partial x_k}(x + \xi_k e_k)\right\vert \\
	\leq& \tilde{C}_4 \epsilon \sum^{m_1}_{\ell=1}\sum^m_{i=1} \left(\abs{a_{ki}} +  \sum^m_{j=1}\abs{ b_{j\ell}a_{kj}}\right)\abs{b_{i\ell}a_{ki}}.
	\end{align*}
	By the triangle inequality and the previous step,  $\norm{\nabla f(x) - \Delta_{\epsilon}[f](x)}_2$ can be bounded by
	\begin{align*}
	&\norm{\nabla f(x) - \Delta_{\epsilon}[f](x)}_2 \leq \tilde{C}_4 \epsilon \left\lbrace \sum^d_{k=1}\left[\sum^{m_1}_{\ell=1}\sum^m_{i=1} \left(\abs{a_{ki}} + \abs{ \sum^m_{j=1} b_{j\ell}a_{kj}}\right)\abs{b_{i\ell}a_{ki}} \right]^2 \right\rbrace^{\frac{1}{2}}\\
	&\leq \tilde{C}_4 \epsilon \left\lbrace \sum^d_{k=1}\left[\sum^{m_1}_{\ell=1}\sum^m_{i=1} \abs{a_{ki}}\abs{b_{i\ell}a_{ki}} \right]^2 \right\rbrace^{\frac{1}{2}} +\tilde{C}_4 \epsilon \left\lbrace \sum^d_{k=1}\left[\sum^{m_1}_{\ell=1}\sum^m_{i,j=1} \abs{b_{j\ell}a_{kj}}\abs{b_{i\ell}a_{ki}} \right]^2 \right\rbrace^{\frac{1}{2}}\\
	&\leq \tilde{C}_4 \epsilon \sum^{m_1}_{\ell=1}\sum^m_{i=1} \abs{b_{i\ell}} \left\lbrace  \sum^d_{k=1} a_{ki}^2 \right\rbrace^{\frac{1}{2}} 
	+\tilde{C}_4 \epsilon \sum^{m_1}_{\ell=1}\sum^m_{i,j=1} \abs{b_{i\ell}b_{j\ell}}\left\lbrace \sum^d_{k=1} a_{kj}^2a_{ki}^2 \right\rbrace^{\frac{1}{2}}\\
	&\leq\tilde{C}_4 \epsilon \sum^{m_1}_{\ell=1}\sum^m_{i=1} \abs{b_{i\ell}} +\tilde{C}_4 \epsilon \sum^{m_1}_{\ell=1}\sum^m_{i,j=1} \abs{b_{i\ell}b_{j\ell}} \\
	&\leq \tilde{C}_4\epsilon m_1 \sqrt{m} + \tilde{C}_4\epsilon m_1 m \leq 2\tilde{C}_4\epsilon m_1 m.
	\end{align*}
	In the last step we used $\sum^m_{i=1}\abs{b_{i\ell}} = \norm{b_{\ell}}_1 \leq \sqrt{m}\norm{b_\ell}_2 = \sqrt{m}$. Setting $C_4 = 2\tilde{C}_4$ finishes the proof.
\end{proof}
\begin{lem}\label{errorhessian}
	Let $\epsilon > 0$, $\norm{x}_2 \leq 1$, then 
	\begin{align}
	\norm{H[f](x) - \Delta^2_{\epsilon}[f](\ve{x})}_F \leq C_5 \epsilon m_1 m^{\frac{3}{2}}
	\end{align}
	for a constant $C_5 > 0$.
\end{lem}
The proof is basically a repetition of the previous one with slightly longer calculations.
\begin{proof}
	Let $k,n \in \set{1,...,d}$ and define $\phi(t) = f(x + t e_k + \epsilon e_n) - f(x + t e_k)$, by the mean value theorem, there exist $0 < \xi_1, \xi_2 < \epsilon$ such that
	\begin{align*}
	(\Delta^2_\epsilon[f](x))_{kn} &= \frac{\phi(\epsilon)-\phi(0)}{\epsilon^2} = \frac{\phi'(\xi_1)}{\epsilon} \\
	&= \frac{\frac{\partial f}{\partial x_k}(x+\xi_1 e_k + \epsilon e_n) - \frac{\partial f}{\partial x_k}(x+\xi_1 e_k)}{\epsilon}\\
	&= \frac{\partial^2 f}{\partial x_k\partial x_n}(x + \xi_1 e_k + \xi_2 e_n).
	\end{align*}
	Hence, we obtain
	\begin{align*}
	\abs{(H[f](x))_{kn} - (\Delta^2_\epsilon[f](x))_{kn}} = \left\vert \frac{\partial^2 f}{\partial x_k\partial x_n}(x) - \frac{\partial^2 f}{\partial x_k\partial x_n}(x + \xi_1 e_k + \xi_2 e_n)\right\vert .
	\end{align*}
	Assume $k,n$ to be fixed and denote $\tilde{x} = x + \xi_1 e_k + \xi_2 e_n$. By recalling our definition of $H[f](x)$ in (\ref{hessians_raw}) follows $\frac{\partial^2 f}{\partial x_k\partial x_n}(x) = \varphi_1(x) + \varphi_2(x)$, where 
	\begin{align*}
	\varphi_1(x) &:= \sum^{m_1}_{\ell=1}\sum^{m}_{i,j=1} h_\ell''(b_\ell^T g(A^T x))g_i'(a_i^T x)g_j'(a_j^T x)a_{ki}a_{nj}b_{i\ell}b_{j\ell}, \\
	\varphi_2(x) &:= \sum^{m_1}_{\ell=1}\sum^m_{i=1}h_\ell'(b_\ell^T g(A^T x))g_i''(a_i^T x) a_{ki}a_{ni}b_{i\ell}.
	\end{align*}
	Thus 
	\begin{align*}
	\abs{(H[f](x))_{kn} - (\Delta^2_\epsilon[f](x))_{kn}} \leq \abs{\varphi_1(x) - \varphi_1(\tilde{x})} + \abs{\varphi_2(x) - \varphi_2(\tilde{x})}.
	\end{align*}
	As before, we start by applying the Lipschitz continuity to the summands of $\abs{\varphi_1(x) - \varphi_1(\tilde{x})}$:
	\begin{align*}
	&\abs{h_\ell''(b_\ell^T g(A^T x))g_i'(a_i^T x)g_j'(a_j^T x) - h_\ell''(b_\ell^T g(A^T \tilde{x}))g_i'(a_i^T \tilde{x})g_j'(a_j^T \tilde{x})} \\
	\leq& \abs{h_\ell''(b_\ell^T g(A^T x))g_i'(a_i^T x)g_j'(a_j^T x) - h_\ell''(b_\ell^T g(A^T x))g_i'(a_i^T \tilde{x})g_j'(a_j^T \tilde{x})} \\
	+& \abs{h_\ell''(b_\ell^T g(A^T x))g_i'(a_i^T \tilde{x})g_j'(a_j^T \tilde{x}) - h_\ell''(b_\ell^T g(A^T \tilde{x}))g_i'(a_i^T \tilde{x})g_j'(a_j^T \tilde{x})} \\ 
	\leq& \eta_2\abs{g_i'(a_i^T x)g_j'(a_j^T x) - g_i'(a_i^T \tilde{x})g_j'(a_j^T \tilde{x})} + \kappa_1^2\abs{h_\ell''(b_\ell^T g(A^T x)) - h_\ell''(b_\ell^T g(A^T \tilde{x}))}\\
	\leq& \eta_2\left[\abs{g_i'(a_i^T x)g_j'(a_j^T x) - g_i'(a_i^T \tilde{x})g_j'(a_j^T x)}  + \abs{g_i'(a_i^T \tilde{x})g_j'(a_j^T x) - g_i'(a_i^T \tilde{x})g_j'(a_j^T\tilde{x} )} \right]\\
	+& \kappa_1^2 \eta_3 \left\vert\sum^{m}_{I=1} b_{I\ell} \left( g_I(a_I^T x) - g_I(a_I^T \tilde{x})\right)\right\vert\\
	\leq& \eta_2 \left[\kappa_1\abs{g_i'(a_i^T x) - g_i'(a_i^T \tilde{x})} + \kappa_1\abs{g_j'(a_j^T x) - g_j'(a_j^T \tilde{x})} \right] + \kappa_1^3 \eta_3 \left\vert\sum^{m}_{I=1} b_{Il}a_I^T(x-\tilde{x})\right\vert \\
	\leq& \eta_2 \kappa_1 \kappa_2\left[\abs{a_i^T(x - \tilde{x})} +\abs{a_j^T(x - \tilde{x})}\right] + \kappa_1^3 \eta_3 \left\vert\sum^{m}_{I=1} b_{I\ell}a_I^T(x-\tilde{x})\right\vert \\
	\leq& \eta_2 \kappa_1 \kappa_2\left[ \abs{ \xi_1 a_{ki} + \xi_2 a_{ni}} + \abs{ \xi_1 a_{kj} + \xi_2 a_{nj}} \right] 
	+ \kappa_1^3 \eta_3 \left\vert \sum^m_{I=1} b_{I\ell}(\xi_1 a_{kI} + \xi_2 a_{nI})\right\vert\\
	\leq& \eta_2 \kappa_1 \kappa_2 \epsilon\left[ \abs{a_{ki}} + \abs{a_{ni}} + \abs{a_{kj}}+ \abs{a_{nj}} \right] 
	+ \kappa_1^3 \eta_3 \epsilon \sum^m_{I=1} \abs{b_{I\ell}}(\abs{a_{kI}} + \abs{a_{nI}})\\
	\leq& \tilde{C}_5 \epsilon \left[ \abs{a_{ki}} + \abs{a_{ni}} + \abs{a_{kj}}+ \abs{a_{nj}} + \sum^m_{I=1} \abs{b_{I\ell}}(\abs{a_{kI}} + \abs{a_{nI}})\right],
	\end{align*}
	where $\tilde{C}_5 = \max\set{ \eta_2 \kappa_1 \kappa_2 ,\kappa_1^3 \eta_3}$. Hence, 
	\begin{align*}
	\abs{\varphi_1(x) - \varphi_1(\tilde{x})} \leq \sum^{m_1}_{l=1}\sum^m_{i,j=1}\tilde{C}_5 \epsilon \left[ \abs{a_{ki}} + \abs{a_{ni}} + \abs{a_{kj}}+ \abs{a_{nj}} + \sum^m_{I=1} \abs{b_{I\ell}}(\abs{a_{kI}} + \abs{a_{nI}})\right]\abs{b_{i\ell}b_{j\ell}a_{ki}a_{nj}}.
	\end{align*}
	Now 
	\begin{align*}
	&\sum^{m_1}_{\ell=1}\sum^m_{i,j=1}\tilde{C}_5\epsilon \left[ \abs{a_{ki}} + \abs{a_{ni}} + \abs{a_{kj}}+ \abs{a_{nj}} \right]\abs{b_{i\ell}b_{j\ell}a_{ki}a_{nj}}\\
	&=\sum^{m_1}_{\ell=1}\sum^m_{i,j=1}\tilde{C}_5 \epsilon \left[ \abs{a_{ki}^2a_{nj}} + \abs{a_{ni}a_{ki}a_{nj}} + \abs{a_{kj}a_{ki}a_{nj}}+ \abs{a_{nj}^2a_{ki}} \right]\abs{b_{i\ell}b_{j\ell}}.
	\end{align*}
	Applying the triangle inequality of the Frobenius norm results in
	\begin{align*}
	&\tilde{C}_5 \epsilon \left( \sum^{d}_{k,n=1} \left[ \sum^{m_1}_{\ell=1}\sum^m_{i,j=1}\left[ \abs{a_{ki}^2a_{nj}} + \abs{a_{ni}a_{ki}a_{nj}} + \abs{a_{kj}a_{ki}a_{nj}}+ \abs{a_{nj}^2a_{ki}} \right]\abs{b_{i\ell}b_{j\ell}} \right]^2\right)^{\frac{1}{2}}\\
	\leq& 2 \tilde{C}_5 \epsilon \left( \sum^{d}_{k,n=1} \left[ \sum^{m_1}_{\ell=1}\sum^m_{i,j=1}\abs{a_{ki}^2a_{nj}} \abs{b_{i\ell}b_{j\ell}} \right]^2\right)^{\frac{1}{2}}
	+ 2 \tilde{C}_5 \epsilon \left( \sum^{d}_{k,n=1} \left[ \sum^{m_1}_{\ell=1}\sum^m_{i,j=1}\abs{a_{ni}a_{ki}a_{nj}} \abs{b_{i\ell}b_{j\ell}} \right]^2\right)^{\frac{1}{2}}\\
	\leq& 2 \tilde{C}_5 \epsilon \sum^{m_1}_{\ell=1}\sum^m_{i,j=1} \abs{b_{i\ell}b_{j\ell}} \left(  \sum^{d}_{k,n=1} \left[ \abs{a_{ki}^2a_{nj}}  \right]^2\right)^{\frac{1}{2}}
	+ 2 \tilde{C}_5 \epsilon \sum^{m_1}_{\ell=1}\sum^m_{i,j=1} \abs{b_{i\ell}b_{j\ell}} \left(  \sum^{d}_{k,n=1} \left[ \abs{a_{ni}a_{ki}a_{nj}}  \right]^2\right)^{\frac{1}{2}}\\
	\end{align*}
	\begin{align*}
	\leq& 2 \tilde{C}_5 \epsilon \sum^{m_1}_{\ell=1}\sum^m_{i=1} \abs{b_{i\ell}}\sum^m_{j=1}\abs{b_{j\ell}} \left\lbrace  \left(  \sum^{d}_{k,n=1} \left[ \abs{a_{ki}^2a_{nj}}  \right]^2\right)^{\frac{1}{2}}
	+\left(  \sum^{d}_{k,n=1} \left[ \abs{a_{ni}a_{ki}a_{nj}}  \right]^2\right)^{\frac{1}{2}}\right\rbrace \\
	\leq& 2 \tilde{C}_5 \epsilon \sum^{m_1}_{\ell=1}\sum^m_{i=1} \abs{b_{i\ell}}\sum^m_{j=1}\abs{b_{j\ell}} \left\lbrace  \left(  \sum^{d}_{k=1} a_{ki}^4 \sum^{d}_{n=1} a_{nj}^2  \right)^{\frac{1}{2}} +
	\left(  \sum^{d}_{k=1} a_{ki}^2 \sum^{d}_{n=1} a_{nj}^2 \right)^{\frac{1}{2}}\right\rbrace \\
	\leq& 4 \tilde{C}_5 \epsilon \sum^{m_1}_{\ell=1}\sum^m_{i=1} \abs{b_{i\ell}}\sum^m_{j=1}\abs{b_{j\ell}}  \norm{a_i}_2 \norm{a_j}_2 \\
	\leq & 4  \tilde{C}_5 \epsilon \sum^{m_1}_{\ell=1} \norm{b_\ell}^2_1\\
	\leq& 4  \tilde{C}_5 \epsilon m_1 m.
	\end{align*}
	The last inequalities are due to $\norm{a_i}_2 = 1$ for all $i = 1,..., m$ and $\norm{b_\ell}_1 \leq \sqrt{m}\norm{b_\ell}_2 = \sqrt{m}$ for all $\ell = 1,..., m_1$. A very similar computation yields
	\begin{align*}
	\tilde{C}_5 \epsilon \left( \sum^{d}_{k,n=1} \left[ \sum^{m_1}_{\ell=1}\sum^m_{i,j=1} \sum^m_{I=1} (\abs{a_{kI}} + \abs{a_{nI}})]\abs{a_{ki}a_{nj}}\abs{ b_{I\ell}b_{i\ell}b_{j\ell}} \right]^2\right)^{\frac{1}{2}} \leq 4\tilde{C}_5 \epsilon m_1 m^{\frac{3}{2}}.
	\end{align*}
	Combining both results gives
	\begin{align*}
	\left\lbrace \sum^{d}_{k,n=1}\left[\abs{\varphi_1(x) - \varphi_1(x + \xi_{1,kn}e_k + \xi_{2, kn}e_n)}\right]^2 \right\rbrace^{\frac{1}{2}} \leq 8\tilde{C}_5 \epsilon m_1 m^{\frac{3}{2}}.
	\end{align*}
	Here we denote $\xi_{1,kn},  \xi_{2, kn}$, to make clear that $\xi_1, \xi_2$ are changing for every partial derivative of second order. However, all $\xi_{1,kn},  \xi_{2, kn}$ are bounded by $\epsilon$, so our result still holds.
	Applying the same procedure to $\abs{\varphi_2(x) - \varphi_2(\tilde{x})}$ yields
	\begin{align*}
	&\abs{h_\ell'(b^T_\ell g(A^T x)) g_i''(a_i^T x) - g_l'(b_\ell g(A^T \tilde{x}))g_i''(a_i^T \tilde{x})} \\
	\leq& \eta_1 \kappa_3 \epsilon ( \abs{a_{ki}} + \abs{a_{ni}}) + \kappa_2 \eta_2 \kappa_1 \epsilon \left\vert \sum^{m_1}_{I=1} b_{I\ell}(\abs{a_{Ik}} + \abs{a_{In}})\right\vert.
	\end{align*}
	By setting $\hat{C}_5 = \max\set{\eta_1\kappa_3, \kappa_1\kappa_2\eta_2}$, we can can develop the same bounds for both parts of the right sum as for $\varphi_1$, and get 
	\begin{align*}
	\left\lbrace \sum^{d}_{k,n=1}\left[\abs{\varphi_2(x) - \varphi_2(x + \xi_{1,kn}e_k + \xi_{2, kn}e_n)}\right]^2 \right\rbrace^{\frac{1}{2}} \leq 8\hat{C}_5 \epsilon m_1 m^{\frac{3}{2}}.
	\end{align*}
	Finally, we get
	\begin{align*}
	&\norm{H[f](x) - \Delta^2_{\epsilon}[f](x)}_F \leq  \left\lbrace \sum^{d}_{k,n=1}\left[\left\vert \frac{\partial^2 f}{\partial x_k\partial x_n}(x) - \frac{\partial^2 f}{\partial x_k\partial x_n}(x + \xi_{1,kn}e_k + \xi_{2, kn}e_n)  \right\vert \right]^2 \right\rbrace^{\frac{1}{2}} \\
	=& \left\lbrace \sum^{d}_{k,n=1}\left[\left\vert \varphi_1(x) + \varphi_2(x) - \varphi_1(x + \xi_{1,kn}e_k + \xi_{2, kn}e_n) - \varphi_2(x + \xi_{1,kn}e_k + \xi_{2, kn}e_n) \right\vert \right]^2 \right\rbrace^{\frac{1}{2}}\\
	\leq& 8\tilde{C}_5\epsilon m_1 m^{\frac{3}{2}} + 8\hat{C}_5\epsilon m_1 m^{\frac{3}{2}}.
	\end{align*}
	Setting $C_5 = 16\max\set{\tilde{C}_5, \hat{C}_5}$ finishes the proof.
\end{proof}
The result is interesting because the error does not depend on $d$, further we did not use the quasi-orthogonality of $A,B$ in any of the calculations, the fact that $\norm{a_i}_2, \norm{b_\ell}_2 \leq 1$ was sufficient.
\subsubsection{Approximation of $L$}
The succeeding theorem extends Theorem \ref{MAINLOG} to finite differences. This extension can also be done with every other bound on $\norm {P_{\hat{L}} - P_{L_{PCA}}}_F$ from the previous section. \\
We can easily extend Algorithm \ref{alg:dimred} to finite differences. Simply replace the matrix 
\begin{align}
M = \left( \opvec(H[f](x_1)) \middle| \dots \middle| \opvec(H[f](x_{m_x})) \right)
\end{align}
by
\begin{align}
\tilde{M} := \left( \opvec(\Delta^2_\epsilon[f](x_1)) \middle| \dots \middle| \opvec(\Delta^2_\epsilon[f](x_{m_x})) \right),
\end{align}
where $\Delta^2_\epsilon[f](x)$ is the finite difference approximation of $H[f](x)$ and $x_1, \dots, x_{m_x}$ are the vectors that were drawn uniformly from the sphere. The result will be the space $\tilde{L}_{PCA}$ spanned by the first $m+m_1$ columns of the left singular vectors of $\tilde{M}$. As previously, we consider the matrix
\begin{align*}
\hat{M} = \left( \opvec(P_L H[f](x_1)) \middle| \dots \middle| \opvec(P_L H[f](x_{m_x})) \right),
\end{align*}
and denote by $\hat{L} \subset L^{vec}$ (cf. (\ref{def_hatM})) the space spanned by the columns of $\hat{M}$.
Let $P_L, P_{\tilde{L}_{PCA}}, P_{\hat{L}}$ be orthogonal projections onto the spaces $L, \tilde{L}_{PCA},\hat{L}$. 

\begin{thm}
	Given the setting above: If Assumption \ref{lowersvbound} holds for $\alpha > 0$, then 
	Algorithm \ref{alg:dimred} applied with finite difference approximations yields $\tilde{L}_{PCA}$ such that, for every $0<t, s\in (0,s_0]$, we have
	\begin{align}\label{eqthm5}
	\norm{P_{\tilde{L}_{PCA}}-P_{\hat{L}}}_F \leq \frac{  2C_5 \epsilon m_1 m^{\frac{3}{2}} + 2C_1\sqrt{(1+t) m_1 \left(\sqrt{\frac{2 \log(m)}{d}} + \frac{1}{d} \right)}}{\sqrt{(1-s)\alpha} -  C_5 \epsilon m_1 m^{\frac{3}{2}}},
	\end{align}
	with probability at least $1 -  2 \exp\left(-2C_3t^2 \frac{m_x}{d}\right) - (m+m_1) \exp\left({-s^2 \frac{m_x \alpha}{ C_2 m_1}}\right)$, where $\epsilon>0$ is the step size used in the finite difference approximation and $s_0 \in (0,1)$ is such that 
	\begin{align}\label{def:s_0}
	\sqrt{(1-s_0)\alpha}  >  C_5 \epsilon m_1 m^{\frac{3}{2}}.
	\end{align}
	The constants $C_1, C_2, C_3, C_5 > 0$ were defined within the previous sections.
\end{thm}
\begin{proof}
	By the proof of Theorem \ref{MAINLOG}, we have
	\begin{align*}
	\norm{M - \hat{M}}_F \leq C_1\sqrt{(1+t)m_x\delta}
	\end{align*}
	for 
	\begin{align*}
	\delta  :=  m_1 \left(\sqrt{\frac{2 \log(m)}{d}} + \frac{1}{d} \right) ,
	\end{align*}
	with probability at least $1 -  2 \exp\left(-2C_3t^2 \frac{m_x}{d}\right)$ ($t>0$). Combining this with the bound on the approximation error from Lemma \ref{errorhessian} yields
	\begin{align*}
	&\norm{\tilde{M} -\hat{M}}_F \leq \norm{M - \tilde{M}}_F + \norm{M - \hat{M}}_F \\
	\leq&    \left\lbrace \sum^{m_x}_{i=1} \norm{H[f](x_i) - \Delta^2_{\epsilon}[f](x_i)}_F^2  \right\rbrace^{\frac{1}{2}} + C_1\sqrt{(1+t)m_x\delta} \\
	\leq&  \left\lbrace \sum^{m_x}_{i=1}  \left( C_5 \epsilon m_1 m^{\frac{3}{2}}\right)^2  \right\rbrace^{\frac{1}{2}} + C_1\sqrt{(1+t)m_x\delta}  \\
	\leq& \sqrt{m_x} C_5 \epsilon m_1 m^{\frac{3}{2}} + C_1\sqrt{(1+t)m_x\delta}, 
	\end{align*}
	with probability at least $1 -  2 \exp\left(-2C_3t^2 \frac{m_x}{d}\right)$.
	Since Assumption \ref{lowersvbound} holds for $\alpha > 0$, we can apply Lemma \ref{boundsv}, such that
	\begin{align*} 
	\sigma_{m+m_1}(M) \geq \sqrt{(1-s)m_x\alpha},
	\end{align*}
	with probability at least $1 - (m+m_1) \exp\left({ \frac{ -s^2 m_x \alpha}{ C_2 m_1}}\right)$. By Weyl's inequality (see Appendix Theorem \ref{weyl}) and given that $\sigma_{m+m_1}(M) \geq \sqrt{(1-s)m_x\alpha}$, we get
	\begin{align}
	\abs{\sigma_{m+m_1}(M) - \sigma_{m+m_1}(\tilde{M}) } &\leq \norm{M - \tilde{M}}_F\\
	&= \sqrt{m_x} C_5 \epsilon m_1 m^{\frac{3}{2}}.
	\end{align}
	By our assumption, $\sqrt{(1-s)\alpha}  >  C_5 \epsilon m_1 m^{\frac{3}{2}}$ for all $s < s_0$ (cf. \ref{def:s_0}), hence
	\begin{align*}
	\sigma_{m+m_1}(\tilde{M}) \geq \sqrt{(1-s)m_x\alpha} - \sqrt{m_x} C_5 \epsilon m_1 m^{\frac{3}{2}},
	\end{align*}
	with probability at least $1 - (m+m_1) \exp\left({ \frac{ -s^2 m_x \alpha}{ C_2 m_1}}\right)$ for all $s \in (0,s_0]$.
	Since the columns of $\hat{M}$ were projected onto a $m+m_1$ dimensional space, we know it has maximal rank $m+m_1$. Hence, $\sigma_{m+m_1+1}(\hat{M}) = 0$ and by the same argument as in  Proposition \ref{MAINWEDIN} of the last chapter, Wedin's bound gives us
	\begin{align*}
	\norm{P_{\hat{L}} - P_{\tilde{L}_{PCA}}} &= \frac{2 \norm{\tilde{M} - \hat{M}}_F}{\abs{\sigma_{m+m_1}(\tilde{M}) - \sigma_{m+m_1+1}(\hat{M})}} \leq \frac{2 \norm{\tilde{M} - \hat{M}}_F}{\sigma_{m+m_1}(\tilde{M})}\\
	&\leq \frac{2\sqrt{m_x} C_5 \epsilon m_1 m^{\frac{3}{2}} + 2C_1\sqrt{(1+t)m_x\delta}}{\sqrt{(1-s)m_x\alpha} - \sqrt{m_x} C_5 \epsilon m_1 m^{\frac{3}{2}}}\\
	&=\frac{ 2C_5 \epsilon m_1 m^{\frac{3}{2}} + 2C_1 \sqrt{(1+t)\delta}}{\sqrt{(1-s)\alpha} -  C_5 \epsilon m_1 m^{\frac{3}{2}}},
	\end{align*}
	with probability at least $1 -  2 \exp\left(-2C_3t^2 \frac{m_x}{d}\right) - (m+m_1) \exp\left({-s^2 \frac{m_x \alpha}{ C_2 m_1}}\right)$.
\end{proof}

==> sections/matrix_subspace/subsection4_dimensionreduction.tex <==
\subsection{Reduction to active subspace}
The Hessians are symmetric, therefore it will suffice to calculate the lower triangle part of $\Delta^2[f](\ve{x})_{\epsilon}$. 
However, one still needs $\mathcal{O}(m_x d^2)$ function evaluations of $f$ to calculate $\Delta_{\epsilon}^2[f](x_1), \dots,  \Delta_{\epsilon}^2[f](x_{m_x})$. 
To circumvent this behavior, we can apply an approach from \cite{forn2}, which allows us to translate our original problem of learning a function in $\mathbb{R}^d$, to learning a representation of that function in $\mathbb{R}^m$. 
The reduction is possible since the active subspace of $f \in \mathcal{F}_d(m_1,m)$ only has dimension $m$. To be more clear: Let $P_{\ma{A}}$ be the orthogonal projection onto the space spanned by $\ve{a}_1, \dots, \ve{a}_m$, then $f(x) = f(P_{\ma{A}}x)$. Once we know $\operatorname{range}(A)$, we can take any orthonormal basis $\ma{\tilde{A}}=(\ve{\tilde{a}}_1 |  \dots | \ve{\tilde{a}}_m )$ of $\operatorname{range}(A)$ and get
\begin{align*}
f(x) = f(P_{\ma{A}}x) = f( \ma{\tilde{A}}\ma{\tilde{A}}^T x ).
\end{align*}
Let $\tilde{f}:\mathbb{R}^m \to \mathbb{R}$ be given by $\tilde{f}(\ve{y}) = f(\ma{\tilde{A}} \ve{y})$ and note that this implies $f(\ve{x}) = \tilde{f}(\ma{\tilde{A}}^T \ve{x})$. By denoting $\ve{\alpha}_i = \ma{\tilde{A}}^T\ve{a}_i$, the function $\tilde{f}$ can also be written as 
\begin{align}\label{defftilde}
\tilde{f}(\ve{y}) = \sum^{m_1}_{\ell=1} h_\ell(\ve{b}_\ell^T \begin{pmatrix}
g_1(\ve{\alpha}_1^T \ve{y})\\
g_2(\ve{\alpha}_2^T \ve{y})\\
\vdots\\
g_m(\ve{\alpha}_m^T \ve{y})
\end{pmatrix}
).
\end{align} 
Hence $\tilde{f}$ has the same form as $f$. 
For the reduction we need to identify $\opspan \left\lbrace \ve{a}_1, \dots, \ve{a}_m \right\rbrace$ or a good approximation of it. Recall that, by (\ref{gradient}),
\begin{align*}
\nabla f(x) \in \opspan \left\lbrace \ve{a}_1, \dots, \ve{a}_m \right\rbrace.
\end{align*}
Therefore we can apply the same algorithm as for the Hessians on the gradients. For $x_1, ..., x_{m_x}$ sampled uniformly from the unit sphere in $\mathbb{R}^d$, denote
\begin{align}
\mathcal{A}&:= \left(\nabla f(x_1)| \dots | \nabla f(x_{m_x}) \right) \in\mathbb{R}^{d \times m_x},\\
\mathcal{\tilde{A}}&:= \left( \Delta_{\epsilon}[f](x_1)| \dots | \Delta_\epsilon[f](x_{m_x}) \right) \in \mathbb{R}^{d \times m_x} .
\end{align}
Further denote by $P_{A},P_{\tilde{A}_{PCA}}$ the projection onto the space spanned by the first $m$ left singular vectors of $\mathcal{A}, \mathcal{\tilde{A}}$. We will assume that $\mathcal{A}$ has full rank, therefore $P_A$ is exactly the projection onto the space $\operatorname{range}(A)$.
\begin{prop}\label{prop:constructspanA}
	If there exists a $\beta> 0$, such that 
	\begin{align}\label{alphaboundgrad}
	\sigma_{m}(\mathbb{E}\left[ \nabla f(X) (\nabla f(X))^T \right]) \geq \beta
	\end{align}
	for $X \sim \Unif(\mathbb{S}^{d-1})$, then with probability at least $1-m\exp(-\frac{s^2 m_x \beta }{2 C_6 m_1})$, we have
	\begin{align}
	\norm{P_A - P_{\tilde{A}_{PCA}}}_F \leq \frac{2 C_4 \epsilon  m_1 m}{\sqrt{(1-s)\beta} - C_4 \epsilon  m_1 m},
	\end{align}
	for all $s \in (0, s_0)$, where $\epsilon>0$ is the step size of the finite difference approximation and $s_0 \in (0,1)$ is such that 
	\begin{align*}
	\sqrt{(1-s_0)\beta} >  C_4 \epsilon  m_1 m.
	\end{align*}
\end{prop}
\begin{proof}
	We start by giving a bound for $\norm{\nabla f(x_i)}_2$. Let $x\in \mathbb{R}^d$ such that $\norm{x}_2 \leq 1$. Then 
	%\color{red}
	%\begin{align*}
	%\norm{\nabla f(x)}_2 & = \norm{\sum^{m_1}_{l=1}\sum^m_{i=1} b_{il} h_l'(b_l^T g(A^T x))g_i'(a_i^T x)a_i  }_2\\
	%&\leq \eta_1 \kappa_1 \norm{\sum^{m_1}_{l=1}\sum^m_{i=1} b_{il}a_i  }_2 = \eta_1 \kappa_1 \norm{\sum^{m_1}_{l=1} A b_l }_2 \\
	%&\leq \eta_1 \kappa_1 \norm{A} \norm{\sum^{m_1}_{l=1} b_l }_2 \leq (1+\epsilon_A) \eta_1 \kappa_1 m_1.
	%\end{align*}
	\begin{align*}
	\norm{\nabla f(x)}_2 & = \norm{\sum^{m_1}_{\ell=1}\sum^m_{i=1} b_{i\ell} h_\ell'(b_\ell^T g(A^T x))g_i'(a_i^T x)a_i  }_2\\
	&= \norm{\sum^{m_1}_{\ell=1}h_\ell'(b_\ell^T g(A^T x))AG_x b_\ell }_2 = \norm{ A G_x B h'(B^T g(A^T x)) }_2 \\
	&\leq (1+\epsilon_{AB})\kappa_1 \norm{h'(B^T g(A^T x))}_2 \leq (1+\epsilon_{AB})\kappa_1 \eta_1 \sqrt{m_1}.
	\end{align*}
	Denote by $P = \bar{A}^T$ the orthogonal projector onto the columns of $\bar{A}$, which denotes the optimal orthogonal matrix of $A$. Then
	\begin{align*}
	\sigma_m(\mathcal{A}) &= \sigma_m(P\mathcal{A}) = \sigma_m(P \mathcal{A}\mathcal{A}^T P^T)^{\frac{1}{2}} \\
	&=\left\lbrace \sum_{i = 1}^{m_x} P\nabla f(x_i) \nabla f(x_i)^T P^T \right\rbrace^{\frac{1}{2}}.
	\end{align*}
	The matrices $P\nabla f(x_i) \nabla f(x_i)^T P^T$ are clearly symmetric and bounded. Thus, 
	\begin{align*}
	\norm{P\nabla f(x_i) \nabla f(x_i)^T P^T} \leq \norm{\nabla f(x_i) \nabla f(x_i)^T}_F \leq \norm{\nabla f(x_i)}^2_2 \leq C_6 m_1,
	\end{align*}
	for $C_6 = (1+\epsilon_{AB})^2\eta_1^2 \kappa_1^2$. Since all $x_i$ are independent and from the same distribution, our assumption (\ref{alphaboundgrad}) yields
	\begin{align*}
	\sigma_m(\mathbb{E} \left[ \sum_{i = 1}^{m_x} P\nabla f(x_i) \nabla f(x_i)^T P^T \right]) \geq m_x \beta.
	\end{align*}
	As in the preceding chapter, we can use the matrix Chernoff inequality (Appendix Theorem \ref{tropp}) to find a lower bound on $\sigma_m(\mathcal{A})$, which holds with high probability, i.e.
	\begin{align*}
	\sigma_m(\mathcal{A}) \geq \sqrt{(1-s)\beta m_x},
	\end{align*}
	with probability at least $1-m\exp(-\frac{s^2 m_x \beta }{2 C_6 m_1})$. Due to Weyl's theorem (Appendix Theorem \ref{weyl}), we then have
	\begin{align}\label{eq:gradientweyl}
	\left| \sigma_m(\mathcal{A})- \sigma_m(\mathcal{\tilde{A}}) \right| \leq \norm {\mathcal{A}-\tilde{\mathcal{A}}}_F .
	\end{align}
	From Lemma \ref{errorgrad} follows
	\begin{align*}
	\norm{\mathcal{A} - \mathcal{\tilde{A}}}_F = \left( \sum^{m_x}_{i=1} \norm{ \nabla f(x_i) - \Delta_{\epsilon}[f](x_i)}_2^2\right)^{\frac{1}{2}}\\
	\leq \sqrt{m_x} C_4 \epsilon  m_1 m.
	\end{align*}
	If our assumption $\sqrt{(1-s_0)\beta} >  C_4 \epsilon  m_1 m$ holds for $s_0 \in (0,1)$, we can combine the results and plug them into (\ref{eq:gradientweyl}):
	\begin{align*}
	\sigma_m(\tilde{\mathcal{A}}) \geq  \sqrt{(1-s)\beta m_x} - \sqrt{m_x} C_4 \epsilon  m_1 m > 0
	\end{align*}
	for all $s \in (0, s_0)$.
	Finally, similar to previous proofs, we can conclude with Wedin's bound (Appendix Theorem \ref{wedin}) that
	\begin{align*}
	\norm{P_{A_{PCA}} - P_{\tilde{A}_{PCA}} }_F  &\leq \frac{\norm{\mathcal{A}- \tilde{\mathcal{A}}}_F}{\left|\sigma_m(\tilde{\mathcal{A}}) - \sigma_{m+1}(\mathcal{A})\right|}\\
	&= \frac{\norm{\mathcal{A}- \tilde{\mathcal{A}}}_F}{\sigma_m(\tilde{\mathcal{A}})}\\
	&\leq \frac{ 2\sqrt{m_x}C_4 \epsilon  m_1 m}{\sqrt{(1-s)m_x\beta} - C_4 \epsilon \sqrt{m_x} m_1 m}\\
	&= \frac{ 2C_4 \epsilon  m_1 m}{\sqrt{(1-s)\beta} - C_4 \epsilon  m_1 m},
	\end{align*}
	with probability at least $1-m\exp(-\frac{s^2 m_x \beta }{2 C_6 m_1})$. The second step is due to the fact that $\mathcal{A}$ has dimension $m$ and therefore $\sigma_{m+1}(\mathcal{A})= 0$.
\end{proof}
The last proposition implies that we are able to approximate $\opspan\set{a_1, ..., a_m}$ given $\beta$ is large enough. Assume that $\norm{P_{A} - P_{\tilde{A}_{PCA}} }_F \leq \delta$ for some small $\delta \in (0,1)$. We can chose any orthonormal basis $\tilde{A}\in \mathbb{R}^{d \times m}$ of $\operatorname{range}(\tilde{A}_{PCA})$ and define $\tilde{f}:\mathbb{R}^m \to \mathbb{R}$ point wise as $\tilde{f}(y) = f(\tilde{A} y)$. We can sample from $\tilde{f}$ at $y$ by evaluating $f(\tilde{A}y)$. Let us summarize the whole procedure:
\color{red} Outcommented because we do not want mymdframe... \color{black}
%\begin{mymdframed}{Reduction to the case $d=m$}
%	Given a function $f\in \mathcal{F}_d(m_1, m)$ (cf. Definition \ref{def:f}):
%	\begin{enumerate}
%		\item Draw $m_x$ vectors $x_1, \dots, x_{m_x}\in \mathbb{R}^d$ from $\Unif(\mathbb{S}^{d-1})$ at random.
%		\item Construct $\tilde{\mathcal{A}} = \left( \Delta_{\epsilon}[f](x_1)| \dots | \Delta_\epsilon[f](x_{m_x}) \right) \in \mathbb{R}^{d\times m_x}$.
%		\item Set ${\tilde{A}_{PCA}}$ to the space spanned by the first $m$ left singular vectors of $\tilde{\mathcal{A}}$.
%		\item Let $\tilde{A} \in \mathbb{R}^{d\times m}$ be the matrix, such that the columns form an orthonormal basis of $\tilde{A}_{PCA}$. Define the function $\tilde{f}:\mathbb{R}^m \to \mathbb{R}$ as $\tilde{f}(y) = f(\tilde{A}^T y)$.
%	\end{enumerate}
%\end{mymdframed}

\begin{thm}\label{reductionisgood}
	Let $f \in \mathcal{F}_d(m_1, m)$ and denote by $\tilde{f}$ the function constructed by the procedure above. Denote by $A,B$ the matrices corresponding to $f$ (cf. chapter \ref{chapter:specification}), and by $\epsilon_A, \epsilon_B, \epsilon_{AB} \geq 0$ the constants from Definition \ref{def:f}.     
	If there exists a $\delta \geq 0$ such that
	\begin{align*}
	\norm{P_A - P_{\tilde{A}_{PCA}}}_F \leq \delta
	\end{align*}
	and
	\begin{align}\label{conditionred}
	0 \leq \sum^{m_1}_{j=1} b_{ij}^2 < 1 - 10\delta - \left( 2 \epsilon_A + 2\epsilon_B +\middle(\epsilon_A +\epsilon_{AB}+\epsilon_{A}\epsilon_{AB}\middle)\frac{1}{1-\epsilon_B} \right) 
	\end{align}
	for all $i = 1,\dots,m$, then 
	\begin{align*}
	\tilde{f} \in \mathcal{F}_m(m_1, m).
	\end{align*}
	
\end{thm}
\begin{proof}
	Since $f\in \mathcal{F}_d(m_1, m)$, it has a representation
	\begin{align*}
	f(x) = \sum^{m_1}_{\ell=1} g(\ve{b}_\ell^T \begin{pmatrix}
	g_1(a_1^T x)\\
	g_2(a_2^T x)\\
	\vdots\\
	g_m(a_m^T x)
	\end{pmatrix}
	).
	\end{align*}
	Hence, $\tilde{f}(y) = f(\tilde{A}^T y)$ can be represented as 
	\begin{align*}
	\tilde{f}(\ve{y}) = \sum^{m_1}_{\ell=1} g(\ve{b}_\ell^T \begin{pmatrix}
	g_1(\ve{\alpha}_1^T \ve{y})\\
	g_2(\ve{\alpha}_2^T \ve{y})\\
	\vdots\\
	g_m(\ve{\alpha}_m^T \ve{y})
	\end{pmatrix}
	).
	\end{align*}
	The functions $g_1, \dots, g_m, h_1, \dots, h_{m_1}$ and the vectors $b_1, \dots, b_{m_1}$ do not change, hence they still fulfill all properties given in Definition \ref{def:f}. Due to the orthogonality of $\tilde{A}$, the length of $\alpha_i$ is bounded, as
	\begin{align*}
	\norm{\alpha_i}_2 = \norm{\tilde{A}^T a_i}_2 \leq \norm{\tilde{A}}\norm{a_i}_2 \leq \norm{a_i}_2 \leq  1,
	\end{align*}
	for all $i=1, \dots, m$.
	Denote $P_{\tilde{A}} = \tilde{A}\tilde{A}^T$ and let $\bar{a}_1, \dots, \bar{a}_m$ be the optimal orthonormal basis w.r.t. $a_1,\dots, a_m$.
	We follow the arguments in \cite[page 9.]{forn2}  and find
	\begin{align*}
	\mathcal{S}(\alpha_1, \dots, \alpha_m) &= \mathcal{S}(\tilde{A}^T a_1, \dots, \tilde{A}^T a_m) = \mathcal{S}(P_{\tilde{A}}a_1, \dots ,P_{\tilde{A}}a_m) \\&\leq (\sum^m_{i=1}\norm{P_{\tilde{A}}a_i - \bar{a}_i}_2^2)^{\frac{1}{2}}\\
	&\leq (\sum^m_{i=1}\norm{P_{\tilde{A}}a_i - \bar{a}_i}_2^2)^{\frac{1}{2}} \\
	&\leq (\sum^m_{i=1}\norm{P_{\tilde{A}}a_i - P_{\tilde{A}}\bar{a}_i}_2^2)^{\frac{1}{2}} + (\sum^m_{i=1}\norm{P_{\tilde{A}}\bar{a}_i - P_{A}\bar{a}_i}_2^2)^{\frac{1}{2}}\\
	&\leq \epsilon_A + \delta.
	\end{align*}
	The condition (\ref{conditionred}) implicitly implies $\delta < \frac{1}{10}$ and $\epsilon_A < \frac{1}{4}$ (otherwise it could not hold). Thus,
	\begin{align}\label{eq:trivialquasiorth}
	\mathcal{S}(\alpha_1, \dots, \alpha_m) \leq \frac{1}{10} + \frac{1}{4} < 1.
	\end{align}
	Let $A^* \in \mathbb{R}^{m\times m}$ be the matrix with columns $\alpha_1, \dots, \alpha_m$. If $\alpha_1, \dots, \alpha_m$ were not independent, then $\oprank(A^*) < m$. 
	Hence, the $m^{th}$ singular value of $A^*$ has to be $0$. By Lemma \ref{opt_orth_mat} follows
	\begin{align*}
	\mathcal{S}(\alpha_1, \dots, \alpha_m) = \left( \sum^m_{i=1} (\sigma_i(A^*) - 1)\right)^{\frac{1}{2}} \geq \abs{\sigma_m (A^*) - 1} \geq 1.
	\end{align*}
	This clearly contradicts (\ref{eq:trivialquasiorth}). Thus,  $\alpha_1, \dots, \alpha_m$ are independent. We checked the length and linear independence of $\alpha_1, \dots, \alpha_m$, which shows that $\tilde{f}$ fulfills the properties 1-5 of the function class $\mathcal{F}_m(m_1, m)$. 
	Denote 
	\begin{align*}
	\epsilon_{A^*} = \mathcal{S}(\alpha_1, \dots, \alpha_m), \hspace{10pt} \epsilon_{A^*B} = \epsilon_{A^*}+\epsilon_{B}+\epsilon_{A^*}\epsilon_{B}.
	\end{align*} 
	Then the application of a series of loose inequalities in combination with $\epsilon_A, \epsilon_B \leq \frac{1}{2}$ yields
	\begin{align*}
	&\left(2 \epsilon_{A^*} + 2\epsilon_B +\middle(\epsilon_{A^*} + \epsilon_{A^*B}+\epsilon_{A^*}\epsilon_{A^*B}\middle)\frac{1}{1-\epsilon_B} \right)\\
	&\leq \left(2 \epsilon_{A}+2\delta + 2\epsilon_B +\middle( 4\delta + \epsilon_{A}  + \epsilon_{AB} +\epsilon_{A}\epsilon_{AB}\middle)\frac{1}{1-\epsilon_B} \right)\\
	&\leq 10\delta + \left(2 \epsilon_{A} + 2\epsilon_B +\middle(  \epsilon_{A}  + \epsilon_{AB} +\epsilon_{A}\epsilon_{AB}\middle)\frac{1}{1-\epsilon_B} \right).
	\end{align*}
	Therefore, under the condition (\ref{conditionred}), $\tilde{f}$ fulfills property 6 of Definition \ref{def:f} and we conclude that $f\in \mathcal{F}_m(m_1,m)$.
\end{proof}
With Theorem \ref{reductionisgood} in mind, a small $\delta$ almost guarantees that the reduced function $\tilde{f}$ will be in $\mathcal{F}_m(m_1,m)$. In this case every result from the previous section is applicable to $\tilde{f}$. Approximations of the directions $\alpha_1, \alpha_2, \dots$ of $\tilde{f}$ can be transformed to approximations of $a_1, a_2, \dots$ by a transformation with the matrix $\tilde{A}$, with an error similar to
\begin{align*}
\norm{\tilde{A} \alpha_i - a_i}_2 &= \norm{\tilde{A}\tilde{A}^T a_i - a_i}_2 = \norm{\tilde{A}\tilde{A}^T a_i - P_A a_i}_2\\
&\leq \norm{\tilde{A}\tilde{A}^T - P_A}_F\norm{a_i}_2 \leq \delta.
\end{align*}
The same works for the vectors corresponding to $v_1,\dots, v_{m_1}$ in the reduced case.

==> sections/section5_numerical_experiments_NNprofiles_old.tex <==
% !TEX root = ../2LayerDraft.tex
\section{Numerical experiments about the recovery of network profiles}
\label{sec:numerical_NNprofiles}
\begin{figure}[t]
\centering
\begin{subfigure}{.5\textwidth}
  \centering
  \includegraphics[width=1.0\linewidth]{img/QO_sig/projection_error}
  \caption{Sigmoid activation function}
  \label{fig:proj_error_sig_qo}
\end{subfigure}%
\begin{subfigure}{.5\textwidth}
  \centering
  \includegraphics[width=1.0\linewidth]{img/QO_tanh/projection_error}
  \caption{$\tanh$ activation function}
  \label{fig:proj_error_tan_qo}
\end{subfigure}
\caption{Error in approximating $\CW$ for perturbed orthogonal weights and
different activation functions.
% For both activation functions, $\Ninnerlayer$ and $m_X$ have little influence, while $\Nouterlayer/\Ninnerlayer$
% affects both cases differently. For sigmoids, increasing $\Nouterlayer/\Ninnerlayer$ increases the error mildly, while for the $\tanh$
% activation increasing $\Nouterlayer/\Ninnerlayer$ results in improved approximation of $\CW(f)$.
}
\label{fig:proj_error_qo}
\end{figure}
In this section we present numerical experiments about the recovery of  network weights
$\{a_i : i \in [\Ninnerlayer]\}$ and $\{v_\ell: \ell\in [\Nouterlayer]\}$ from few point
queries of the network.
% \marginpar{\TKchallenge{We could add an algorithmic procedure here as a summary?}}
The recovery procedure leverages the theoretical insights that have been provided in previous sections. We neglect the active subspace reduction
and concentrate on the case $d = \Ninnerlayer$.
We construct an approximation $P_{\hat \CW} \approx P_{\CW}$ using Algorithm
\ref{alg:approximation_matrix_space}. Then we randomly generate a number of matrices
$\{M^k_0: k \in [K]\} \in \hat \CW \cap \bbS$, and compute the sequences
$M^k_{j+1} = F_{\gamma}(M_j^k)$ as in Algorithm \ref{alg:approximation_neural_network_profiles}.
For each limiting matrix $\{M_{\infty}^{k}: k \in [K]\}$,
we compute the largest eigenvector $u_1(M_{\infty}^{k})$, and then
cluster $\{u_1(M_{\infty}^{k}): k \in [K]\}$ into $\Ninnerlayer + \Nouterlayer$ classes using kMeans++.
After projecting the resulting cluster centers onto $\bbS^{d-1}$, we obtain vectors
$\{\hat w_j: j\in [\Ninnerlayer + \Nouterlayer]\}$ that are used as approximations to  $\{a_i: i\in [\Ninnerlayer]\}$
and $\{v_\ell: \ell \in[\Nouterlayer]\}$.


We perform experiments for different scenarios, where either the activation function,
or the construction of the network weights varies. Guided by our theoretical results,
we pay particular attention to how the network architecture, \emph{e.g.}, $\Ninnerlayer$ and $\Nouterlayer$,
influences the simulation results. The entire procedure is rather flexible and can be adjusted in different ways, {\it e.g.} changing the
distribution $\mu_X$. To provide a fair account of the success, we fix
hyperparameters of the approach throughout all experiments. Test scenarios, hyperparameters,
and error measures are reported below in more detail. Afterwards, we present and discuss the results.
\begin{figure}
\centering
\begin{subfigure}{.5\textwidth}
  \centering
  \includegraphics[width=0.75\linewidth]{img/QO_sig/post_kNN_fp_rate}
  \caption{False positives, sigmoid activation function}
  \label{fig:fp_sig_qo}
\end{subfigure}%
\begin{subfigure}{.5\textwidth}
  \centering
  \includegraphics[width=0.75\linewidth]{img/QO_tanh/post_kNN_fp_rate}
  \caption{False positives, $\tanh$ activation function}
  \label{fig:fp_tanh_qo}
\end{subfigure}
\begin{subfigure}{.5\textwidth}
  \centering
  \includegraphics[width=1.0\linewidth]{img/QO_sig/percentage_recovered_separate}
  \caption{Recovery rates, sigmoid activation function }
  \label{fig:recov_sig_qo}
\end{subfigure}%
\begin{subfigure}{.5\textwidth}
  \centering
  \includegraphics[width=1.0\linewidth]{img/QO_tanh/percentage_recovered_separate}
  \caption{Recovery  rates, $\tanh$ activation function}
  \label{fig:recov_tanh_qo}
\end{subfigure}
\caption{False positive and recovery rates for perturbed orthogonal weights and for different activation functions.
% In both cases increasing $\Ninnerlayer$ consistently reduces the false positive rate and increases the recovery rate.
% Increasing $\Nouterlayer$ on the other hand influences the results negatively for the sigmoid function, and positively
% for the $\tanh$ activation.
}
\label{fig:fp_recov_qo}
\end{figure}
\paragraph{Scenarios and construction of the networks}
The network is constructed by choosing activation functions and network weights
$\{a_i : i \in [\Ninnerlayer]\}$, $\{b_\ell : \ell \in  [\Nouterlayer]\}$, and $v_\ell$ is then
defined via $v_\ell = \frac{AG_0 b_\ell}{\N{AG_0 b_\ell}_2}$, see Definition \ref{def:f}. To construct activation functions,
we set $g_i(t) = \phi(t + \theta_i)$ for $i \in [\Ninnerlayer]$, and $h_\ell(t) = \phi(t + \tau_\ell)$
for $\ell \in [\Nouterlayer]$. We choose either $\phi(t) = \tanh(t)$, or
$\phi(t) = \frac{1}{1+e^{-t}} - \frac{1}{2}$ (shifted sigmoid function), and sample offsets $\theta_i$, $\tau_\ell$ independently at random
from $\CN(0,0.01)$.

We test two different scenarios for the weights. In the first case we sample them independently from $\Uni{\bbS^{\Ninnerlayer-1}}$.
The second scenario models both $\{a_i : i \in [\Ninnerlayer]\}$ and $\{b_\ell : \ell \in  [\Nouterlayer]\}$
as perturbed orthogonal systems. To construct these, we first sample orthogonal bases uniformly at random,
and then apply a random perturbation. The perturbation is such that $(\sum_{i=1}^{\Ninnerlayer}(\sigma_i(A) - 1)^2)^{-1/2} \approx (\sum_{i=1}^{\Nouterlayer}(\sigma_i(B) - 1)^2)^{-1/2} \approx  0.3$, where $\sigma_i(A)$ and $\sigma_i(B)$ denote singular values of $A$ and $B$.
\paragraph{Hyperparameters}
Unless stated differently, we sample $m_X = 1000$ Hessian locations from $\mu_X = \sqrt{\Ninnerlayer}\textrm{Uni}\left(\bbS^{\Ninnerlayer-1}\right)$,
and use $\epsilon = 10^{-5}$ in the finite difference approximation \eqref{def:finite_differences_hessian}.
We generate $1000$ random matrices $\{M_0^k: k \in [1000]\}$ by sampling $m^k \sim \CN(0,\Id_{\Ninnerlayer + \Nouterlayer})$,
and by defining $M_0^k := \bbP_{\bbS}(\sum_{i=1}^{\Ninnerlayer + \Nouterlayer}m_i^k u_i)$, where the $u_i$'s
are as in Algorithm \ref{alg:approximation_matrix_space}. The constant $\gamma = 2$
{is used in the definition of $\Fiter$, and the iteration is stopped if $\lambda_1(M_{j+1}^k) - \lambda_1(M_{j}^k) < 10^{-5}$, or after 200 iterations.
kMeans++ is run with default settings using \textit{sklearn}. All reported results are
averages over 30 repetitions.}

% We note here that choosing $m_X > 1000$ always increased the performance mildly,
% but the benefit is rather small compared to the additional computational power required.
% Revisiting Theorem \ref{thm:approx_space_bound}, this is because the second nonlinear layer
% adds a bias term that prevents $P_{\hat \CW} \rightarrow P_{\CW}$ in the case $m_X \rightarrow \infty$.
% We also comment that the sampling strategy can have positive and negative influence on the results. Choosing
% for example $\mu_X = \textrm{Uni}\left(\bbS^{\Ninnerlayer-1}\right)$ mostly led to worse performance,
% while choosing $\mu_X = R\textrm{Uni}\left(\bbS^{\Ninnerlayer-1}\right)$ with $R \sim \Uni{[1,\sqrt{m_0}]}$
% seems a viable alternative if $m_X$ is choosen sufficiently large. Since we
% are interested in a uniform scheme, we do not try to maximize the benefit of $\mu_X$ in our experiments.

\paragraph{Error measures}
Three error measures are reported:
\begin{itemize}
\item the normalized projection error $\frac{\Vert \hat P_{\CW} - P_{\CW}\Vert_F^2}{\Ninnerlayer + \Nouterlayer}$,
\item a false positive rate $\textrm{FP}(T)=\frac{\#\{j : E(\hat w_j) > T\}}{\Ninnerlayer + \Nouterlayer}$,
where $T>0$ is a threshold, and $E(u)$ is defined by,
% \begin{align*}
% E(u) := \min\left\{\min_{\substack{i=1,\ldots,\Ninnerlayer,\  s = \pm 1}}\N{s a_i - u}^2, \min_{\substack{i=1,\ldots,\Nouterlayer \\ s = \pm 1}}\N{s v_i - u}^2\right\}.
% \end{align*}
\begin{align*}
E(u) := \min_{v \in \{\pm a_i,\pm v_\ell : i \in [\Ninnerlayer],\ell \in [\Nouterlayer]\}}\N{u - v}^2_2,
\end{align*}
\item recovery rate $\textrm{R}_a(T) = \frac{\#\{i : \CE(a_i) < T\}}{\Ninnerlayer}$, and $\textrm{R}_v(T) = \frac{\#\{i : \CE(v_i) < T\}}{\Nouterlayer}$, where
{
\begin{align*}
\CE(u) &:= \min_{v \in \{\pm \hat  w_j : j \in [\Ninnerlayer+\Nouterlayer] \}}\N{u - v}^2_2.
\end{align*}}
\end{itemize}
% Firstly, we compute the projection error $\Vert \hat P_{\CW} - P_{\CW}\Vert_F^2$ normalized
% by $\Ninnerlayer + \Nouterlayer$. Secondly, we compute a false positive rate \emph{FP}$(T)=\frac{\#\{l : E(c_l) > T\}}{\Ninnerlayer + \Nouterlayer}$,
% where $T$ is a threshold parameter, and $E(c_l)$ is defined by
% \begin{align*}
% E(u) := \min\left\{\min_{\substack{i=1,\ldots,\Ninnerlayer \\ s \in \{-1,1\}}}\N{s a_i - u}^2, \min_{\substack{i=1,\ldots,\Nouterlayer \\ s \in \{-1,1\}}}\N{s v_i - u}^2\right\}.
% \end{align*}
% Lastly, we report the recovery rates for each layer, given by
% \begin{align*}
% \textrm{R}_{a}(T) &= \frac{\#\{i : \CE(a_i) < T\}}{\Ninnerlayer},\quad \textrm{R}_{v}(T) = \frac{\#\{i : \CE(v_i) < T\}}{\Nouterlayer},
% \textrm{ with } \CE(u) &:= \min_{\substack{l=1,\ldots,\Ninnerlayer + \Nouterlayer \\ s \in \{-1,1\}}}\N{s u - c_l}^2.
% \end{align*}
\paragraph{Results for perturbed orthogonal weights}
\label{subsec:exp_perturbed_orthogonal_weights}
\begin{figure}[t]
\centering
\begin{subfigure}{.5\textwidth}
  \centering
  \includegraphics[width=1.0\linewidth]{img/uni_sig/projection_error}
  \caption{Sigmoid activation function}
  \label{fig:proj_error_sig_uni}
\end{subfigure}%
\begin{subfigure}{.5\textwidth}
  \centering
  \includegraphics[width=1.0\linewidth]{img/uni_tanh/projection_error}
  \caption{$\tanh$ activation function}
  \label{fig:proj_error_tan_uni}
\end{subfigure}
\caption{Error in approximating $\CW$ for weights sampled independently from the unit sphere, and for different
activation functions.
% For both activation functions, $\Ninnerlayer$ and $m_X$ have little influence, while $\Nouterlayer/\Ninnerlayer$
% affects both cases differently. For sigmoids, increasing $\Nouterlayer/\Ninnerlayer$ increases the error significantly, while for the $\tanh$
% activation increasing $\Nouterlayer/\Ninnerlayer$ results in improved approximation of $\CW(f)$.
}
\label{fig:proj_error_uni}
\end{figure}
\begin{figure}
\centering
\begin{subfigure}{.5\textwidth}
  \centering
  \includegraphics[width=0.75\linewidth]{img/uni_sig/post_kNN_fp_rate}
  \caption{False positives, sigmoid activation function}
  \label{fig:fp_sig_uni}
\end{subfigure}%
\begin{subfigure}{.5\textwidth}
  \centering
  \includegraphics[width=0.75\linewidth]{img/uni_tanh/post_kNN_fp_rate}
  \caption{False positives, $\tanh$ activation function}
  \label{fig:fp_tanh_uni}
\end{subfigure}
\begin{subfigure}{.5\textwidth}
  \centering
  \includegraphics[width=1.0\linewidth]{img/uni_sig/percentage_recovered_separate}
  \caption{Recovery rates, sigmoid activation function}
  \label{fig:recov_sig_uni}
\end{subfigure}%
\begin{subfigure}{.5\textwidth}
  \centering
  \includegraphics[width=1.0\linewidth]{img/uni_tanh/percentage_recovered_separate}
  \caption{Recovery rates, $\tanh$ activation function}
  \label{fig:recov_tanh_uni}
\end{subfigure}
\caption{False positive and recovery rates for weights sampled uniformly at random from the unit-sphere
and for different activation functions.
% In both cases increasing $\Ninnerlayer$ consistently reduces the false positive rate and increases the recovery rate.
% Increasing $\Nouterlayer$ on the other hand influences the results negatively for the sigmoid function, and positively
% for the $\tanh$ activation.
}
\label{fig:fp_recov_uni}
\end{figure}
The results of the study are presented in Figures \ref{fig:proj_error_qo}
and \ref{fig:fp_recov_qo}, and show that our procedure can be used to recover
many of the network weights, while suffering only few false positives.
Considering for example a sigmoidal network,
we have almost perfect recovery of the weights in both
layers at a threshold of $T = 0.05$ for any network architecture, see Figures \ref{fig:fp_sig_qo}, \ref{fig:recov_sig_qo}. For
a $\tanh$-network, the performance is slightly worse, but we still recover
most weights in the second layer, and a large portion in the
first layer at a reasonable threshold, see Figures \ref{fig:fp_tanh_qo}, \ref{fig:recov_tanh_qo}.

Inspecting the plots more closely, we can notice some shared trends and differences between
sigmoid- and $\tanh$-networks. In both cases, the
performance improves when increasing the number of neurons in the first layer, even though the
number of weights that need to be recovered increases accordingly. This is particularly the case
for $\tanh$-networks as visualized in Figures \ref{fig:fp_tanh_qo} and \ref{fig:recov_tanh_qo},
and is most likely caused by reduced correlation of the weights in higher dimensions. The correlation
is encoded within the frame constant $\nu$ used in the  analysis in Section \ref{sec:individual_and_assignment}.

For fixed $\Ninnerlayer$ on the other hand, different activation functions react differently to changes of $\Nouterlayer$.
Considering a sigmoid network, the projection error increases,
and the recovery of weights in the second layer worsens as shown in Figures \ref{fig:proj_error_sig_qo} and \ref{fig:recov_sig_qo}. This is
expected by Theorem \ref{thm:approx_space_bound}.
Inspecting the results for $\tanh$-networks, the projection
error actually decreases when increasing $\Nouterlayer$, see Figure \ref{fig:proj_error_tan_qo},
and the recovery performance gets better. Figure \ref{fig:recov_tanh_qo} shows
that especially weights in the first layer are more easily recovered if
$\Nouterlayer$ is large, such that the case $\Ninnerlayer = 45$, $\Nouterlayer = 23$ allows for
perfect recovery at a threshold $T = 0.05$. This behavior can not be explained by our general
theory, e.g. Theorem \ref{thm:approx_space_bound}.
% It is however
% an interesting future avenue to perform similar analysis while concentrating on
% specific networks only in order to theoretically understand how the difference between sigmoid and $\tanh$-network
% can be explained.
\paragraph{Results for random weights from the unit-sphere.}
When sampling the weights independently from the unit-sphere, the recovery problem seems more challenging
for both activation functions, and all network architectures. Figures
\ref{fig:recov_sig_uni} and \ref{fig:recov_tanh_uni} suggest that especially recovering the
weights of the second layer is more difficult than in the perturbed orthogonal case.
Still, we achieve good performance in many cases. For sigmoid networks, Figure \ref{fig:recov_sig_uni} shows that
we always recover most weights in the first layer, and a large portion of weights
in the second layer if $\Nouterlayer/\Ninnerlayer$ is small. Moreover, keeping $\Nouterlayer/\Ninnerlayer$ constant while increasing $\Ninnerlayer$
improves the performance significantly. Figures \ref{fig:fp_sig_uni}, \ref{fig:recov_sig_uni} show almost perfect recovery for
$\Ninnerlayer = 45,\ \Nouterlayer = 5$ with suffering only few false positives.

For $\tanh$-networks, Figure \ref{fig:recov_tanh_uni} shows that increasing $\Ninnerlayer$
benefits recovery of weights in both layers, while increasing $\Nouterlayer$ benefits
recovery of first layer weights and harms recovery of second layer weights. We still achieve
small false positive rates in Figure \ref{fig:fp_tanh_uni}, and good recovery for $\Ninnerlayer = 45$,
and the trend continues when further increasing $\Ninnerlayer$.

{Finally, a notable difference between the perturbed orthogonal case and the unit-sphere case is the behavior of the projection error $\|P_{\hat \CW}- P_{\CW}\|_F/(\Ninnerlayer+\Nouterlayer)$ for networks with sigmoid activation function. Comparing Figures
\ref{fig:proj_error_sig_qo} and \ref{fig:proj_error_sig_uni}, the dependency of the projection error on $\Nouterlayer$ is stronger when sampling independently from the unit-sphere.
This is explained by Theorem \ref{thm:approx_space_bound} since $\N{B}^2$ is independent of $\Nouterlayer$ in the perturbed orthogonal case, and grows like $\mathcal{O}(\sqrt{\Nouterlayer})$ when sampling from the unit-sphere.}


==> sections/subsections/subsec_4_largest_eigenvec.tex <==
% !TEX root = ../../Ridge.tex
\subsection{Largest eigenvectors of almost rank one matrices}
\label{subsec:largest_eigenvectors_nn_profiles}
% In this part we conclude the proof of the main result of this section, that is
% we show that the largest eigenvector of a local maximizer with large eigenvalue
% is close to one of the neural network profiles $w_i$.
Recall that $\Lriesz$ is the lower Riesz constant of the system $\{w_1\otimes w_1,\ldots, w_m \otimes w_m\}$.
\begin{lem}
\label{lem:largest_eigenvector}
Let $M \in \hat \CW \cap \bbS$ with spectral decomposition $M = \sum_{i=1}^{d}\lambda_i u_i \otimes u_i$, ordered according to $\lambda_1 >\lambda_2 \geq \ldots \geq \lambda_d$. Assume $\max\{\Perror,\Ferror\}\leq 1/4$. If $\Delta := \lambda_1 - \lambda_2 > \Ferror + 2 \Perror$, then
\begin{align}
\min_{j=1,\ldots,m}\N{w_{j} - u_1} \leq \sqrt{8}\frac{\Lriesz^{-1/2}\sqrt{\Ferror} + \Perror}{\Delta - \Ferror - 2\Perror}.
\end{align}
\end{lem}
\begin{proof}
We can represent $M$ in terms of the basis elements of $\hat W$ by $M = \sum_{i=1}^{m}\sigma_i \hat W_i$, and denote by
$Z \in \CW$ the matrix satisfying $M = P_{\hat  W}(Z)$. \textcolor{red}{Furthermore, let $\sigma_{j^*} = \max_j \sigma_j > 0$ where the
positivity follows from Lemma \ref{lem:max_sigma_pos}.}
Using $Z = \sum_{i=1}^{m}\sigma_i w_i \otimes w_i$ and $\N{Z}_F \leq (1-\Perror)^{-1}$, we first notice that
\begin{equation}
\label{eq:lambda_1_lower_bound}
\begin{aligned}
\lambda_1 &= \left\langle M, u_1 \otimes u_1\right\rangle = \left\langle Z, u_1 \otimes u_1\right\rangle + \left\langle M-Z, u_1 \otimes u_1\right\rangle\\
&\leq \sum_{i=1}^{m}\sigma_i \left\langle w_i, u_1\right\rangle^2 + \N{M - Z}_F \leq \sigma_{j^*} \Uframe + 2\Perror \leq \sigma_{j^*} + \Ferror + 2\Perror,
\end{aligned}
\end{equation}
hence $\sigma_{j^*} \geq \lambda_1 - \nu - 2\delta$.
Now we want to use Theorem \ref{thm:davis_kaham_thm2} (Davis-Kahan Theorem) to compare $M$ with a matrix for which the largest eigenvector is given by $w_{j^*}$.
Using the notation in Theorem \ref{thm:davis_kaham_thm2}, we let $A = \sigma_{j^*} w_{j^*} \otimes w_{j^*}$, $B = M$, $S_1 = [\infty, \sigma_{j^*}]$, and
$S_2 = [\lambda_2, -\infty]$. Since $P_{B}(S_2) = \Id - u_1 \otimes u_1$ and
\begin{align*}
\N{w_{j^*} - u_1}^2 &= 2(1 - \left\langle w_{j^*},u_1\right\rangle) \leq 2(1 - \left\langle w_{j^*},u_1\right\rangle^2) =2(1 - \N{(\Id - P_{B}(S_2))w_{j^*}}^2) \\
&= 2\N{P_{B}(S_2)w_{j^*}}^2 =2\N{P_{B}(S_2)w_{j^*}\otimes w_{j^*}}_F^2 = 2\N{P_{A}(S_1)P_{B}(S_2)}_F^2
\end{align*}
we can use Theorem \ref{thm:davis_kaham_thm2} to get
\begin{align}
\label{eq:first_bound_wj_u1}
\N{w_{j^*} - u_1} &=  \sqrt{2}\N{P_{A}(S_1)P_{B}(S_2)}_F \leq \sqrt{2}\frac{\N{P_{A}(S_1)(A - B)P_{B}(S_2)}_F}{\sigma_j^* - \lambda_2}
\leq  \sqrt{2}\frac{\N{P_{A}(S_1)(A - B)}_F}{\sigma_j^* - \lambda_2}.
\end{align}
To further bound $\N{P_{A}(S_1)(A - B)}_F$, we first decompose
% Then we obtain for for $P_{A}(S_1) = w_{j^*}\otimes w_{j^*}$ and $P_{B}(S_2) = \Id - u_1\otimes u_1$
% \begin{align*}
% \N{w_{j^*}^T P_{M}(S_2)}_2 =  \N{w_{j^*} \otimes w_{j^*}P_{M}(S_2)}_F = \N{P_{A}(S_1)P_{B}(S_2)}_F\leq \frac{\N{P_{A}(S_1)(A - B)P_{B}(S_2)}_F}{\sigma_j^* - \lambda_2}.
% \end{align*}
\[
\N{P_{A}(S_1)(A - B)}_F = \N{P_{A}(S_1)(A - M)}_F \leq \N{P_{A}(S_1)(A - Z)}_F + \Perror/(1-\Perror)
\]
and then use $A = \sigma_{j^*}w_{j^*}\otimes w_{j^*}$ and $P_{A}(S_1) = w_{j^*}\otimes w_{j^*}$ to get
\begin{align*}
\N{P_{A}(S_1)(A - Z)}_F &= \N{\sum\limits_{j\neq j^*}\sigma_j P_{A}(S_1)(w_j \otimes w_j)} = \N{\sum\limits_{j\neq j^*}\sigma_j \left\langle w_{j^*}, w_j\right\rangle w_j \otimes w_{j^*}}\\
&\leq \sum\limits_{j\neq j^*}\SN{\sigma_j} \SN{\left\langle w_{j^*}, w_j\right\rangle} \leq \N{\sigma}_2 \sqrt{\sum\limits_{j\neq j^*}\left\langle w_{j^*}, w_j\right\rangle^2} \leq \N{\sigma}_2 \sqrt{\Ferror}.
\end{align*}
Combining this with \eqref{eq:first_bound_wj_u1}, $\delta/(1-\delta)\leq 2\delta$, and $\sigma_j^* > \lambda_1 - \nu - 2\delta$, we obtain
\begin{align*}
\N{w_{j^*} - u_1} \leq \sqrt{2}\frac{\N{\sigma}_2 \sqrt{\Ferror}+ 2\Perror}{\lambda_1 - \Ferror - 2\Perror - \lambda_2} =
\sqrt{2}\frac{\N{\sigma}_2 \sqrt{\Ferror}+ 2\Perror}{\Delta - \Ferror - 2\Perror}.
% \N{w_{j^*}^T P_{M}(S_2)}_2  \leq \frac{\N{\sigma}_2\sqrt{\Ferror} + 2\Perror}{\lambda_1 - \lambda_2 - \Ferror - 2\Perror} \leq \frac{2\Lriesz^{-1/2}\sqrt{\Ferror} + 2\Perror}{\Delta - \Ferror - 2\Perror}.
\end{align*}
The result follows since $\{w_i \otimes w_i\}_{i=1,\ldots,m}$ is a Riesz basis
and thus $\N{\sigma}_2 \leq \Lriesz^{-1/2}\N{Z}_F \leq 2\Lriesz^{-1/2}$.
\end{proof}

% Now, denote the eigendecomposition $M^* = \sigma_{j^*}w_{j^*}\otimes w_{j^*}+ \sum_{i=1}^{D-1} \gamma_i v_i \otimes v_i$. Since
% \[
% 1 = \N{M}_F^2 = \sum_{i=1}^{D} \lambda_i^2 = \lambda_1^2 + \sum_{i=2}^{D} \lambda_i^2 \geq 1 - c\nu + \CO(\nu^2)+ \sum_{i=2}^{D} \lambda_i^2 \Rightarrow \max_{i=2,\ldots,D} \lambda_i^2 \leq c\nu + \CO(\nu^2)
% \]
% \marginpar{\TKchallenge{Insert Davis Kahan/Wedin's statement in appendix at the end.}}
% Weyl's Theorem then implies that $M^*$ has at least $D-1$ eigenvalues bounded by $(2+c)\nu + \CO(\nu^2)$. Since
% the assumption on $\nu$ on the other hand implies
% $\sigma_{j^*} \geq 1 - (2+c)\nu + \CO(\nu^2) > (2+c)\nu + \CO(\nu^2)$, it follows that $\max_{i}\gamma_i \leq (2+c)\nu + \CO(\nu^2)$,
% and $\sigma_{j^*}$ is the largest eigenvalue of $M^*$.
% We can now use the Davis Kahan Theorem to compare the maximum eigenvector of $M^*$, given by $w_{j^*}$, to the maximum eigenvector of $M$, given by $u_1$. More precisely, let $P_{\parallel} = u_1\otimes u_1$, $P_{\perp} = \Id - P_{\parallel}$. Then
% \begin{align*}
% \N{ P_{\perp} w_{j^*}}  = \N{ P_{\perp}P_{w_{j^*}\otimes w_{j^*}}} &\leq \frac{\N{M-M^*}_F}{\sigma_{j^*} - \min_{i=2,\ldots,D}\lambda_i} \leq \frac{2\nu + \CO(\nu^2)}{1 - 2(1+c)\nu} + \CO(\nu^2).
% \end{align*}
% This implies the result for $\N{w_{j^*} - u_1}$ since
% \begin{align*}
% \N{w_{j^*} - u_1}^2 &= 2(1 - \left\langle w_{j^*},u_1\right\rangle) \leq 2(1 - \left\langle w_{j^*},u_1\right\rangle^2)\\
% &=2(1 - \N{(\Id - P_{M}(S_2))w_{j^*}}^2)= 2\N{P_{M}(S_2)w_{j^*}}^2.
% \end{align*}
% \end{proof}
% \noindent
% The proof of Theorem \ref{thm:main_theorem_individual_recovery} follows finally as
% a Corollary of the results gathered in Section \ref{sec:individual_and_assignment}.
% \begin{proof}[Proof of Theorem \ref{thm:main_theorem_individual_recovery}]
% Let $X_{\infty} = \sum_{i=1}^{D}\lambda_i^{\infty}u_i^{\infty}\otimes u_i^{\infty}$ denote the resulting matrix of Algorithm \ref{alg:approximation_neural_network_profiles}
% with $\lambda_1^{\infty}$ satisfying the assumptions. Since $\lambda_1^{\infty} > 1/\sqrt{2}$, we have
% $\N{M} = \lambda_1^{\infty} > \lambda_2^{\infty}$. Then,
% Lemma \ref{lem:iteration_and_stopping_condition} first implies $X_{\infty} = (\lambda_{1}^{\infty})^{-1} P_{\hat \CW}(u_1^{\infty} \otimes u_1^{\infty})$,
% and  Theorem \ref{thm:characterization_local_maximizer} implies $X_{\infty}$
% is a local maximizer of \eqref{eq:nonlinear_program}. Moreover, Theorem \ref{thm:lower_bound_eigenvalue} boosts the eigenvalue to
% $\lambda_1^2 > 1 - 18\nu + \CO(\nu^2)$. Finally, we notice that
% $2(2+18)\nu + \CO(\nu^2) = 40\nu + \CO(\nu^2)< 72\nu + \CO(\nu^2) < 1$, therefore Lemma \ref{lem:largest_eigenvector}
% can be applied and the result follows.
% \end{proof}


==> sections/subsections/subsec_62_v1.tex <==
% !TEX root = ../../2LayerDraft.tex

\subsection{\textcolor{blue}{OLD GD:} Reconstructing the network function using gradient descent}
\label{subsec:reconstructing_f}
The previous section allows to assign unlabeled candidates $\{\hat w_i : i \in [\Ninnerlayer + \Nouterlayer]\}$
to either the first or second layer, resulting in matrices
$\hat A = [\hat a_1|\ldots|\hat a_{\Ninnerlayer}]$ and $\hat V = [\hat v_1|\ldots|\hat v_{\Nouterlayer}]$
that ideally approximate $A$ and $V$ up to column signs and permutations. Assuming the network $f \in \CF(\Ninnerlayer,\Ninnerlayer, \Nouterlayer)$
is generated by a universal activation function, i.e. $g_i(t) = \phi(t + \theta_i)$ and $h_\ell(t) = \phi(t + \tau_{\ell})$
for some $\phi$, this means only signs, permutations, and bias
vectors $\theta \in \bbR^{\Ninnerlayer}$, $\tau \in \bbR^{\Nouterlayer}$ are missing to reconstruct $f$.

Let now $\CD_{m}$ denote the set of $m\times m$ diagonal matrices, and define
a parameter space $\Omega := \CD_{\Ninnerlayer}\times \CD_{\Nouterlayer} \times \bbR^{\Ninnerlayer}\times \bbR^{\Nouterlayer}$.
To reconstruct the original network $f$, we propose to fit parameters $(D_1, D_2, w, z) \in \Omega$ of a function $\hat f: \bbR^{\Ninnerlayer}\times \Omega  \rightarrow \bbR$
defined by
\begin{align*}
\hat f(x;D_1, D_2, w, z) &= 1^\top\phi(D_2 \hat B^\top \phi(D_1 \hat A^\top x + w) + z),\quad
\textrm{with}\quad \hat b_\ell:=  \frac{\diag\left(\left(\phi'(w)\right)^{-1}\right)D_1\hat A^{-1}\hat v_\ell}{\N{\diag\left(\left(\phi'(w)\right)^{-1}\right) D_1 \hat A^{-1}\hat v_\ell}},
\end{align*}
to a number of additionally queried points $\{(X_i,Y_i) : i \in [m_f]\}$
where $Y_i = f(X_i)$ and $X_i \sim \CN(0,\Id_{\Ninnerlayer})$. This can be written
as solving the optimal program
\begin{equation}
\label{eq:recover_network_functional}
\min_{(D_1, D_2, w, z) \in \Omega}
J(D_1,D_2, w, z):=\sum_{i=1}^{m_f}\left(Y_i - \hat f(X_i;D_1, D_2, w, z)\right)^2.
\end{equation}
We note that $\dim(\Omega) = 2\Ninnerlayer + 2\Nouterlayer$, which implies
that the optimal program has significantly fewer free parameters compared to
the entire network itself. This is because we made use of precomputed matrices $\hat A$
and $\hat V$. We will now show in the next Proposition that there exists parameters $(D_1, D_2, w, z) \in \Omega$
that allow for exact recovery of the original network, whenever $\hat A$ and $\hat V$
are correct up to signs and permutation. The proof requires only elementary linear algebra,
and properties of sign and permutation matrices. Details are deferred to the Appendix.

\begin{prop}
\label{prop:representation_f}
Let $f \in \CF(\Ninnerlayer,\Ninnerlayer, \Nouterlayer)$ with $g_i(t) = \phi(t + \theta_i)$ and $h_\ell(t) = \phi(t + \tau_{\ell})$.
If there exist sign matrices $S_A$, $S_V$, and permutations $\pi_A$,
$\pi_V$ such that  $A\pi_A = \hat A S_A$, $V\pi_V = \hat V S_V$, we have
$f(x) = \hat f(x; S_A, S_V, \pi_A^\top \theta, \pi_V^\top \tau)$.
% \begin{align*}
% f(x) &= 1^\top\phi(S_V \hat B^\top \phi(S_A \hat A^\top x + \hat \theta) + \hat \tau),\quad \textrm{where}\quad \hat B_\ell:=  \frac{\diag\left(\left(\phi'(\hat \theta)\right)^{-1}\right)S_A\hat A^{-1}\hat V_\ell}{\N{\diag\left(\left(\phi'(\hat \theta)\right)^{-1}\right) S_A \hat A^{-1}\hat V_\ell}}.
% \end{align*}
\end{prop}
\begin{proof}[Proof of Proposition \ref{prop:representation_f}]
\textcolor{blue}{TK: Should be moved to Appendix, but didn't want to interfere with the files!}
The first step is to replace first layer weights $A$ by $\hat A S_A$. This can be achieved
by injecting the permutation $\pi_A$ in the first layer. Specifically we get
\begin{align}
\label{eq:repara_f_1}
f(x) &= 1^\top \phi(B^\top \phi(A^\top x + \theta) + \tau) = 1^\top \phi(B^\top \pi_A \phi((A\pi_A)^\top x + \pi_A^\top \theta) + \tau) \\
&=1^\top \phi((\pi_A^\top B)^\top \phi(S_A A^\top x + \pi_A^\top \theta) + \tau).
\end{align}
Next we need to replace the matrix $\pi_A^\top B$ using $V$ respectively $\hat V$. Let
$n \in \bbR^{\Nouterlayer}$ be defined as $n_\ell = \N{AGb_\ell}^{-1}$, and $N = \diag(n)$. By definition
we have $V = AGBN$, implying the relation $B =  G^{-1}A^{-1}V N^{-1}$. Using
$A = \hat A S_A \pi_A^\top$, $V = \hat VS_V\pi_V^\top$, $S_A^{-1} = S_A$, and $\pi_A^{-1} = \pi_A^\top$, it follows that
\begin{align*}
\pi_A^\top B = \pi_A^\top G^{-1} \pi_A S_A \hat A^{-1} \hat V S_V \pi_V^\top N^{-1} = (\pi_A^\top G \pi_A)^{-1} S_A \hat A^{-1} \hat V S_V \pi_V^\top N^{-1}
\end{align*}
Now, since $G = \diag(\phi'(\theta))$, we have $\pi_A^\top G \pi_A = \diag(\pi_A^\top(\phi'(\theta))) = \diag(\phi'(\pi_A^\top\theta))=:\tilde G$.
Inserting into \eqref{eq:repara_f_1}, we get
\begin{align*}
f(x) &=1^\top \phi(N^{-1} \pi_V S_V \hat V^\top \hat A^{-\top} S_A \tilde G^{-1} \phi(S_A A^\top x + \pi_A^\top \theta) + \tau)
\end{align*}
Furthermore, since the dot product with $1$ is permutation invariant, we can permute the activation of the second layer with $\pi_V^\top$. Then,
using that $\tilde N = \pi_V^\top N \pi_V$ is diagonal, and thus commutes with $S_V$, we get
\begin{align*}
f(x) & =1^\top \phi(\tilde N S_V \hat V^\top \hat A^{-\top} S_A \tilde G^{-1} \phi(S_A A^\top x + \pi_A^\top \theta) + \pi_V^\top \tau) \\
&= 1^\top \phi(\tilde N^{-1} S_V \hat V^\top \hat A^{-\top} S_A \tilde G^{-1} \phi(S_A A^\top x + \pi_A^\top \theta) + \pi_V^\top \tau)\\
&= 1^\top \phi(S_V \tilde N^{-1}  \hat V^\top \hat A^{-\top} S_A \tilde G^{-1} \phi(S_A A^\top x + \pi_A^\top \theta) + \pi_V^\top \tau).
\end{align*}
It remains to show that $\hat B = \tilde G^{-1}  S_A \hat A^{-1} \hat V \tilde N^{-1}$, which is implied if $\tilde N$
is a diagonal matrix with $\tilde N_{ll} = \Vert \tilde G S_A \hat A^{-1}\hat v_\ell\Vert$.
Clearly $\tilde N$ is a diagonal matrix since $\tilde N = \pi_V^\top N \pi_V = \diag(\pi_V^\top n)$.
Furthermore, the normalization $\N{b_\ell} = 1$ (see Definition \ref{def:f}) and $B =  G^{-1}A^{-1}V N^{-1}$ imply
\begin{align*}
1 = \N{b_\ell} = \frac{\N{G^{-1}A^{-1}v_\ell}}{n_\ell}\quad \textrm{ and thus }\quad n_\ell = \N{G^{-1}A^{-1}v_\ell}.
\end{align*}
Using this, and $A^{-1} = \pi_A S_A \hat A^{-1}$, $V \pi_V = \hat V S_V$, we obtain
\begin{align*}
\tilde N &= \diag(\pi_V^\top n) = \diag\left(\pi_V^\top\left(\N{G^{-1}A^{-1}v_1},\ldots,\N{G^{-1}A^{-1}v_{\Nouterlayer}}\right)\right)\\
&=\diag\left(\N{G^{-1}A^{-1}(V\pi_V)_1},\ldots,\N{G^{-1}A^{-1}(V\pi_V)_{\Nouterlayer}}\right)\\
&=\diag\left(\N{G^{-1}\pi_A S_A \hat A^{-1}(\hat V S_V)_1},\ldots,\N{G^{-1}\pi_A S_A \hat A^{-1}(\hat V S_V)_{\Nouterlayer}}\right)\\
&=\diag\left(\N{G^{-1}\pi_A S_A \hat A^{-1}\hat v_1},\ldots,\N{G^{-1}\pi_A S_A \hat A^{-1}\hat v_{\Nouterlayer}}\right),
\end{align*}
where we used that $S_V$ is only each column of $\hat V$ by $\pm 1$. The result follows since $\pi_A^\top$
is orthogonal, so it can be inserted from the left into the norm, and we can replace $\pi_A^\top G^{-1}\pi_A = \tilde G^{-1}$.
\end{proof}
\begin{rem}[Simplification for odd functions]
\label{rem:prop_simplification_odd_functions}
If $\phi$ in Proposition \eqref{prop:representation_f} satisfies $\phi(-t) = -\phi(t)$,
then $\hat f(x; S D_1, D_2, S w, z) = \hat f(x; D_1, D_2, w, z)$ for arbitrary
sign matrix $S$. Thus, choosing $S = S_A$, it follows that
$f(x) = \hat f(x; \Id_{\Ninnerlayer}, S_V, S_A \pi_A^\top w, \pi_V^\top \tau)$.
\end{rem}

Assuming $\hat A$ and $\hat V$ are correct up to sign and permutation,
Proposition \ref{prop:representation_f} implies that $J = 0$ is the global optimum,
and it is attained by parameters leading to the original network $f$.
Furthermore Remark \ref{rem:new_prop_simplification_odd_functions} implies that there is ambiguity
with respect to $D_1$, if $\phi$ is an odd function. Thus
we can also prescribe $D_1 = \Id_{\Ninnerlayer}$ and neglect optimizing over $D_1$ if $\phi$ is odd.

We now study feasibility of \eqref{eq:recover_network_functional}  with extensive numeric tests.
To assess the performance isolated from
error propagation in the entire pipeline, we first consider the case when
$\hat A = A$ and $\hat V = V$ is prescribed. Afterwards we present results
for $\hat A \approx A$ and $\hat V \approx V$.


% \begin{table}
% 	\begin{center}
% 		\begin{tabular}{ccccccc}
% 			\hline
% 			& \multicolumn{3}{c}{$\Ninnerlayer = 30$} & \multicolumn{3}{c}{$\Ninnerlayer = 45$}\\
% 			\hline
% 			Scenario & $\Nouterlayer =  3$ & $\Nouterlayer = 9$ & $\Nouterlayer = 15$ & $\Nouterlayer = 5$ & $\Nouterlayer = 14$ & $\Nouterlayer = 23$\\
% 			\hline
% 			& MSE,\ \  $E_{\infty}$ & MSE,\ \  $E_{\infty}$ & MSE,\ \  $E_{\infty}$ & MSE,\ \  $E_{\infty}$ & MSE,\ \  $E_{\infty}$ & MSE,\ \  $E_{\infty}$\\
% 			& Failed  & Failed  & Failed  & Failed  & Failed  & Failed  \\ \\ \hline
% 			POD/sig\\
% 			Pipeline & $0.9$, $7.8$ & $0.9$, $6.4$ & $9.5$, $27.8$ & $1.8$, $8.1$ & $1.1$, $6.3$ & $12.4$, $41.1$\\
% 			 & $17$ & $31$ & $45$ & $17$ & $10$ & $72$ \\
% 			$\hat A,\hat V = A,V$ & $<0.1$, $1.5$ & $0.2$, $2.0$ & $0.7$, $4.6$ & $<0.1$, $1.7$ & $0.2$, $2.2$ & $5.9$, $23.5$\\
%  			 & 0 & 0 & 3 & 0 & 0 & 0 \\ \\ \hline
% 			 POD/$\tanh$\\
%  			Pipeline & $11.1$, $52.3$ & $4.0$, $21.6$ & $1.1$, $12.0$ & $12.4$, $57.8$ & $4.3$, $18.5$ & $0.7$, $9.8$\\
%  			 & $53$ & $43$ & $13$ & $93$ & $30$ & $0$ \\
%  			$\hat A,\hat V = A,V$ & \multicolumn{6}{c}{All errors $<0.1$}\\
%   			 &  \multicolumn{6}{c}{ No failed cases} \\ \\ \hline
% 			$\bbS^{\Ninnerlayer - 1}$/sig\\
%  			% All & $12.5$, $56.0$ & $4.5$, $21.3$ & $1.7$, $14.2$ & $18.3$, $52.2$ & $0.8$, $10.1$ & $0.8$, $9.8$\\
%  			%  & $70$ & $57$ & $3$ & $93$ & $43$ & $0$ \\
%  			$\hat A,\hat V = A,V$ & $1.8$, $8.4$ & $0.8$, $8.2$ & $2.3$, $14.0$ & $0.5$, $5.5$ & $1.0$, $9.0$ & $2.2$, $16.0$\\
%   			 & $6$ & $0$ & $0$ & $0$ & $0$ & $3$ \\ \\
% 			\hline
% 			$\bbS^{\Ninnerlayer - 1}$/$\tanh$\\
%  			% All & $12.5$, $56.0$ & $4.5$, $21.3$ & $1.7$, $14.2$ & $18.3$, $52.2$ & $0.8$, $10.1$ & $0.8$, $9.8$\\
%  			%  & $70$ & $57$ & $3$ & $93$ & $43$ & $0$ \\
%  			$\hat A,\hat V = A,V$ & $<0.1$, $0.2$ & $1.1$, $3.5$ & $0.7$, $4$ & $<0.1$, $<0.1$ & $<0.1$, $<0.1$ & $<0.1$, $0.3$\\
%   			 & \multicolumn{6}{c}{ No failed cases} \\ \\ \hline
% 		\end{tabular}
% 	\end{center}
% 	\caption{Mean squared error (MSE) and $L_{\infty}$-error ($E_{\infty}$) of the reconstructed network using \eqref{eq:recover_network_functional}.
% 	All values represent percentages. We consider a trial as failed if $MSE > 20\%$. The scenarios correspond to those
% 	in Sections \ref{sec:numerical_NNprofiles} and \ref{subsec:distinguishing}. Pipeline indicates that we use $\hat A$ and $\hat V$
% 	by previously described methods. Otherwise we run \eqref{eq:recover_network_functional} with $A = \hat A$ and $V = \hat V$.}
% 	\label{tab:function_learning_results}
% \end{table}
%
%
% \begin{table}
% 	\begin{center}
% 		\begin{tabular}{ccccccc}
% 			\hline
% 			& \multicolumn{3}{c}{$\Ninnerlayer = 30$} & \multicolumn{3}{c}{$\Ninnerlayer = 45$}\\
% 			\hline
% 			Scenario & $\Nouterlayer =  3$ & $\Nouterlayer = 9$ & $\Nouterlayer = 15$ & $\Nouterlayer = 5$ & $\Nouterlayer = 14$ & $\Nouterlayer = 23$\\
% 			\hline
% 			& MSE,\ \  $E_{\infty}$ & MSE,\ \  $E_{\infty}$ & MSE,\ \  $E_{\infty}$ & MSE,\ \  $E_{\infty}$ & MSE,\ \  $E_{\infty}$ & MSE,\ \  $E_{\infty}$\\
% 			& Failed  & Failed  & Failed  & Failed  & Failed  & Failed  \\ \\ \hline
% 			POD/sig\\
% 			Pipeline & $1.2$, $7.9$ & $0.5$, $7.2$ & $1.2$, $11.7$ & $1.1$, $6.1$ & $0.3$, $6.0$ & $10.4$, $28.0$\\
% 			 & $24$ & $20$ & $17$ & $34$ & $10$ & $17$ \\
% 			$\hat A,\hat V = A,V$ & $<0.1$, $0.2$ & $<0.1$, $0.1$ & $<0.1$, $<0.1$ & $<0.1$, $0.2$ & $<0.1$, $<0.1$ & $1.8$, $11.1$\\
%  			 & \multicolumn{6}{c}{ No failed cases} \\ \\ \hline
% 			 POD/$\tanh$\\
%  			Pipeline & $-$, $-$ & $3.6$, $20.0$ & $2.0$, $15.8$ & $-$, $-$ & $3.0$, $18.1$ & $1.7$, $14.0$\\
%  			 & $100$ & $56$ & $13$ & $100$ & $40$ & $0$ \\
%  			$\hat A,\hat V = A,V$ & \multicolumn{6}{c}{All errors $<0.1$}\\
%   			 &  \multicolumn{6}{c}{ No failed cases} \\ \\ \hline
% 			$\bbS^{\Ninnerlayer - 1}$/sig\\
%  			% All & $12.5$, $56.0$ & $4.5$, $21.3$ & $1.7$, $14.2$ & $18.3$, $52.2$ & $0.8$, $10.1$ & $0.8$, $9.8$\\
%  			%  & $70$ & $57$ & $3$ & $93$ & $43$ & $0$ \\
%  			$\hat A,\hat V = A,V$ & $<0.1$, $0.3$ & $<0.1$, $0.1$ & $<0.1$, $<0.1$ & $<0.1$, $0.2$ & $<0.1$, $0.1$ & $1.3$, $10.7$\\
%   			 & \multicolumn{6}{c}{ No failed cases} \\ \\
% 			\hline
% 			$\bbS^{\Ninnerlayer - 1}$/$\tanh$\\
%  			% All & $12.5$, $56.0$ & $4.5$, $21.3$ & $1.7$, $14.2$ & $18.3$, $52.2$ & $0.8$, $10.1$ & $0.8$, $9.8$\\
%  			%  & $70$ & $57$ & $3$ & $93$ & $43$ & $0$ \\
%  			$\hat A,\hat V = A,V$ & \multicolumn{6}{c}{All errors $<0.1$}\\
%   			 & \multicolumn{6}{c}{ No failed cases} \\ \\ \hline
% 		\end{tabular}
% 	\end{center}
% 	\caption{Mean squared error (MSE) and $L_{\infty}$-error ($E_{\infty}$) of the reconstructed network using \eqref{eq:recover_network_functional}
% 	while fixing $D = \Id_{\Ninnerlayer}$. For description of the Table see Table \ref{tab:function_learning_results}.}
% 	\label{tab:function_learning_results_woSa}
% \end{table}

\paragraph{Numerical experiments}
\begin{table}
	\begin{center}
		\begin{tabular}{cccccccc}
			\hline
			& & \multicolumn{3}{c}{$\Ninnerlayer = 30$} & \multicolumn{3}{c}{$\Ninnerlayer = 45$}\\
			\hline
			Scenario & & $\Nouterlayer =  3$ & $\Nouterlayer = 9$ & $\Nouterlayer = 15$ & $\Nouterlayer = 5$ & $\Nouterlayer = 14$ & $\Nouterlayer = 23$\\ \hline
POD/sig & MSE & $2.1e^{-4}$ & $1.5e^{-3}$ & $1.4e^{-2}$ & $2.6e^{-4}$ & $1.5e^{-3}$ & $5.9e^{-2}$ \\
       & $E_{\infty}$ & $1.5e^{-2}$ & $2.0e^{-1}$ & $6.0e^{-2}$ & $1.7e^{-2}$ & $2.2e^{-2}$ & $2.4e^{-1}$\\ \hline
POD/$\tanh$ & MSE & $8.4e^{-7}$ & $\approx 0$ & $\approx 0$ & $5.9e^{-8}$ & $\approx 0$ & $\approx 0$\\
       & $E_{\infty}$ & $6.0e^{-4}$ & $7.9e^{-8}$ & $\approx 0$ & $2.0e^{-4}$ & $1.3e^{-9}$ & $\approx 0$\\ \hline
$\bbS^{\Ninnerlayer-1}$/sig & MSE & $5.6e^{-2}$ & $8.5e^{-3}$ & $2.3e^{-2}$ & $4.6e^{-3}$ & $1.0e^{-2}$ & $2.9e{-2}$\\
       & $E_{\infty}$ & $1.4e^{-1}$ & $8.3e^{-2}$ & $1.4e^{-1}$ & $5.5e^{-2}$ & $9.0e^{-2}$ & $1.7e^{-1}$\\ \hline
$\bbS^{\Ninnerlayer-1}$/$\tanh$ & MSE & $4.4e^{-6}$ & $1.1e^{-2}$ & $7.0e^{-2}$ & $4.0e^{-8}$ & $1.9e^{-14}$ & $2.2e^{-4}$\\
       & $E_{\infty}$ & $2.3e^{-3}$ & $3.5e^{-2}$ & $4.0e^{-2}$ & $1.8e^{-4}$ & $9.0e^{-8}$ & $3.0e^{-3}$\\ \hline
 			% % All & $12.5$, $56.0$ & $4.5$, $21.3$ & $1.7$, $14.2$ & $18.3$, $52.2$ & $0.8$, $10.1$ & $0.8$, $9.8$\\
 			% %  & $70$ & $57$ & $3$ & $93$ & $43$ & $0$ \\
 			% 	$\bbS^{\Ninnerlayer - 1}$/sig & & $<0.1$, $0.5$ & $<0.1$, $0.6$ & $<0.1$, $0.8$ & $<0.1$, $0.4$ & $<0.1$, $0.6$ & $<0.1$, $0.9$\\
			% \hline
 			% % All & $12.5$, $56.0$ & $4.5$, $21.3$ & $1.7$, $14.2$ & $18.3$, $52.2$ & $0.8$, $10.1$ & $0.8$, $9.8$\\
 			% %  & $70$ & $57$ & $3$ & $93$ & $43$ & $0$ \\
 			% 	$\bbS^{\Ninnerlayer - 1}$/$\tanh$ & & \multicolumn{6}{c}{All errors $<0.1$}\\ \hline
		\end{tabular}
	\end{center}
	\caption{Errors of the reconstructed network using \eqref{eq:recover_network_functional}
  when prescribing $\hat A = A$ and $\hat V = V$. The scenarios correspond to those in Sections \ref{sec:numerical_NNprofiles} and \ref{subsec:distinguishing}.}
	\label{tab:old_function_learning_results}
\end{table}


\begin{table}
	\begin{center}
		\begin{tabular}{cccccccc}
			\hline
			& & \multicolumn{3}{c}{$\Ninnerlayer = 30$} & \multicolumn{3}{c}{$\Ninnerlayer = 45$}\\
			\hline
			Scenario & & $\Nouterlayer =  3$ & $\Nouterlayer = 9$ & $\Nouterlayer = 15$ & $\Nouterlayer = 5$ & $\Nouterlayer = 14$ & $\Nouterlayer = 23$\\ \hline
POD/sig & MSE & $3.7e^{-4}$ & $1.0e^{-1}$ & $2.0e^{-1}$ & $3.7e^{-4}$ & $1.1e^{-2}$ & $2.4e^{-1}$ \\
       & $E_{\infty}$ & $2.2e^{-2}$ & $2.2e^{-1}$ & $4.1e^{-1}$ & $2.0e^{-2}$ & $6.3e^{-2}$ & $5.0e^{-1}$\\
       & Trials [$\%$] & $55$ & $82$ & $86$ & $59$ & $90$ & $83$\\ \hline
POD/$\tanh$ & MSE & $-$ & $6.1e^{-3}$ & $3.0e^{-2}$ & $-$ & $3.8e^{-3}$ & $7.6e^{-3}$\\
       & $E_{\infty}$ &  $-$ & $9.4e^{-2}$ & $1.4e^{-1}$ & $-$ & $7.6e^{-2}$ & $9.8e^{-2}$ \\
       & Trials [$\%$] & $0$ & $27$ & $73$ & $0$ & $37$ & $100$\\ \hline
 			% % All & $12.5$, $56.0$ & $4.5$, $21.3$ & $1.7$, $14.2$ & $18.3$, $52.2$ & $0.8$, $10.1$ & $0.8$, $9.8$\\
 			% %  & $70$ & $57$ & $3$ & $93$ & $43$ & $0$ \\
 			% 	$\bbS^{\Ninnerlayer - 1}$/sig & & $<0.1$, $0.5$ & $<0.1$, $0.6$ & $<0.1$, $0.8$ & $<0.1$, $0.4$ & $<0.1$, $0.6$ & $<0.1$, $0.9$\\
			% \hline
 			% % All & $12.5$, $56.0$ & $4.5$, $21.3$ & $1.7$, $14.2$ & $18.3$, $52.2$ & $0.8$, $10.1$ & $0.8$, $9.8$\\
 			% %  & $70$ & $57$ & $3$ & $93$ & $43$ & $0$ \\
 			% 	$\bbS^{\Ninnerlayer - 1}$/$\tanh$ & & \multicolumn{6}{c}{All errors $<0.1$}\\ \hline
		\end{tabular}
	\end{center}
	\caption{Errors of the reconstructed network using \eqref{eq:recover_network_functional}
  when using approximated $\hat A \approx A$ and $\hat V \approx V$. Trials indicates the percentage of repititions
  where $\hat A$ and $\hat V$ satisfy \eqref{eq:trial_condition}. The scenarios correspond to those in Sections \ref{sec:numerical_NNprofiles} and \ref{subsec:distinguishing}.}
	\label{tab:old_function_learning_results_approx_A_V}.
\end{table}

We minimize \eqref{eq:recover_network_functional} with standard gradient descent and
learning rate $1$ if $\phi(t) = \frac{1}{1+e^{-t}} - 1/2$ (shifted sigmoid),
respectively learning rate $0.025$ if $\phi(t) = \tanh(t)$. We sample $m_f = 10(\Ninnerlayer + \Nouterlayer)$
additional points according to $X_i \sim \CN(0,\Id_{\Ninnerlayer})$.
Gradient descent is run for 500K iterations (due to small number of variables,
this is not time consuming), and only prematurely stopped if the iteration stalls. All variables
are initialized with draws from $\CN(0,0.1)$.

Denoting $\omega^* = (D_1^*, D_2^*, D_3^*, w^*, z^*) \in \Omega$ as the gradient descent output, we measure
the relative mean squared error (MSE) and the relative $L_{\infty}$-error
\[
\textrm{MSE} = \frac{\sum_{i=1}^{m_{\textrm{test}}} (\hat f(Z_i;\omega^*) - f(Z_i))^2}{\sum_{i=1}^{m_{\textrm{test}}}f(Z_i)^2},\quad
\textrm{E}_{\infty} = \frac{\max_{i \in [m_{\textrm{test}}]}\SN{f(Z_i;\omega^*) - f(Z_i)}}{\max_{i \in [m_{\textrm{test}}]}\SN{f(Z_i)}},
\]
using $m_{\textrm{test}} = 50000$ samples $Z_i \sim \CN(0,\Id_{\Ninnerlayer})$.

Table \ref{tab:old_function_learning_results} presents the results of the experiments and
shows that we reconstruct a network function that is very close to the original network $f$
in both $L_2$ and $L_{\infty}$ norm in many scenarios. Often we even achieve errors that
are close to zero (or can be driven that far by using more gradient descent iterations),
implying that we indeed reconstruct a network which is uniformly close to $f$.
In some cases, primarily with sigmoid activation, the $E_{\infty}$ error remains
around $\approx 10^{-1}$, indicating that gradient descent converges to a local minima which may not
be a function uniformly close to $f$.
% Table \ref{tab:function_learning_results} summarizes the results of the study. For
% the cases $\hat A = A$ and $\hat V = V$, minimizing \eqref{eq:new_GD_recover_network_functional}
% with $m_f = 10(\Ninnerlayer + \Nouterlayer)$ additional points achieves convincing
% performance since both the $L_2$-error and $L_{\infty}$-error become small. In many of
% these trials, the errors are actually close to machine precision, or can be driven that far
% by using additional GD-iterations, or higher learning rates. This suggests that the minimization
% indeed recovers the original network function. On the other hand, Table \ref{tab:function_learning_results} also shows that
% \eqref{eq:new_GD_recover_network_functional} is quite sensitive towards $\hat A$ and $\hat V$ because the
% number of failed trials increases significantly if we instead use approximated $\hat A$ and $\hat V$.
% It is also in accordance with results of Sections \ref{sec:numerical_NNprofiles}
% and \ref{subsec:distinguishing} that learning the function is easier for $\tanh$ activation
% (sigmoid activation) if $m_1$ increases (decreases).
We also tested \eqref{eq:new_GD_recover_network_functional} when fixing $D = \Id_{\Ninnerlayer}$
since $\tanh$ and the shifted sigmoid are odd functions, and thus Remark \ref{rem:prop_simplification_odd_functions}
applies. The results are qualitatively similar to those in Table \ref{tab:old_function_learning_results},
but quantitatively improve the error in some cases by up to three orders of magnitude.
Still, the maximal $E_{\infty}$ error remains around $10^{-1}$ for sigmoid networks with $\Ninnerlayer = 45$
and $\Nouterlayer = 23$.

Finally, we ran similar experiments for perturbed orthogonal weights and when using $\hat A$ and $\hat V$ precomputed with methods
that have been described in Sections \ref{sec:numerical_NNprofiles} and \ref{subsec:distinguishing}.
The quality of the results varies dependent on if $\hat A \approx A$ and $\hat V \approx V$
(up to sign and permutation) holds, or whether a fraction of the weights has not been
recovered. To isolate cases where $\hat A \approx A$ and $\hat V \approx V$
holds, we report averaged MSE and $L_{\infty}$ over all trials satisfying
\begin{equation}
\label{eq:trial_condition}
\sum_{i=1}^{\Ninnerlayer}\CE(a_i) +  \sum_{\ell = 1}^{\Nouterlayer}\CE(v_{\ell})  < 0.5,\quad \textrm{(see Section \ref{sec:numerical_NNprofiles} for the Definition of } \CE),
\end{equation}
and additionally the percentage of trials satisfying this condition. The results in
Table \ref{tab:old_function_learning_results_approx_A_V} show that the reconstructed function still
approximates the original function, even if the weights are only approximately correct.
Therefore we conclude that that minimizing \eqref{eq:new_GD_recover_network_functional} provides
a very efficient way to learn the remaining network structure from just few point samples,
once entangled network weights $A$ and $V$ are (approximately) known.




% Table \ref{tab:function_learning_results} summarizes the results of the study. For
% the cases $\hat A = A$ and $\hat V = V$, minimizing \eqref{eq:recover_network_functional}
% with $m_f = 10(\Ninnerlayer + \Nouterlayer)$ additional points achieves convincing
% performance since both the $L_2$-error and $L_{\infty}$-error become small. In many of
% these trials, the errors are actually close to machine precision, or can be driven that far
% by using additional GD-iterations, or higher learning rates. This suggests that the minimization
% indeed recovers the original network function. On the other hand, Table \ref{tab:function_learning_results} also shows that
% \eqref{eq:recover_network_functional} is quite sensitive towards $\hat A$ and $\hat V$ because the
% number of failed trials increases significantly if we instead use approximated $\hat A$ and $\hat V$.
% It is also in accordance with results of Sections \ref{sec:numerical_NNprofiles}
% and \ref{subsec:distinguishing} that learning the function is easier for $\tanh$ activation
% (sigmoid activation) if $m_1$ increases (decreases).
%
% We also tested \eqref{eq:recover_network_functional} when fixing $D = \Id_{\Ninnerlayer}$
% since both activation functions we test are odd functions, and thus Remark \ref{rem:prop_simplification_odd_functions}
% applies. Table \ref{tab:function_learning_results_woSa} shows that this further
% improves the performance when using $\hat A = A$ and $\hat V = V$,
% but can have detrimental effect in the approximate cases.
%
% \newpage
%
%
% Let $\CD_{m}$ denote the set of $m\times m$ diagonal matrices.
% We now want to propose an optimal program over $2(\Ninnerlayer + \Nouterlayer)$
% variables to find the missing network pieces. The following proposition shows how $f$
% can be reparametrized to make use of $\hat A$ and $\hat V$.
% The proof of the proposition is technical but requires only elementary linear algebra,
% and properties of sign and permutation matrices. Details are deferred to the Appendix.
%
%
% \begin{prop}
% \label{prop:representation_f}
% Let $f \in \CF(\Ninnerlayer,\Ninnerlayer, \Nouterlayer)$ with $g_i(t) = \phi(t + \theta_i)$ and $h_\ell(t) = \phi(t + \tau_{\ell})$, and define
% the function $\hat f: \bbR^{\Ninnerlayer}\times \CD_{\Nouterlayer}
% \times \CD_{\Ninnerlayer} \times \bbR^{\Nouterlayer} \times \bbR^{\Ninnerlayer} \rightarrow \bbR$ via
% \begin{align*}
% \hat f(x;D, D', w, z) &= 1^\top\phi(D' \hat B^\top \phi(D \hat A^\top x + w) + z),\quad
% \textrm{with}\quad \hat b_\ell:=  \frac{\diag\left(\left(\phi'(w)\right)^{-1}\right)D\hat A^{-1}\hat v_\ell}{\N{\diag\left(\left(\phi'(w)\right)^{-1}\right) D \hat A^{-1}\hat v_\ell}}.
% \end{align*}
% If there exist sign matrices $S_A$, $S_V$, and permutations $\pi_A$,
% $\pi_V$ such that  $A\pi_A = \hat A S_A$, $V\pi_V = \hat V S_V$, we have
% $f(x) = \hat f(x; S_A, S_V, \pi_A^\top \theta, \pi_V^\top \tau)$.
% % \begin{align*}
% % f(x) &= 1^\top\phi(S_V \hat B^\top \phi(S_A \hat A^\top x + \hat \theta) + \hat \tau),\quad \textrm{where}\quad \hat B_\ell:=  \frac{\diag\left(\left(\phi'(\hat \theta)\right)^{-1}\right)S_A\hat A^{-1}\hat V_\ell}{\N{\diag\left(\left(\phi'(\hat \theta)\right)^{-1}\right) S_A \hat A^{-1}\hat V_\ell}}.
% % \end{align*}
% \end{prop}
% \begin{proof}[Proof of Proposition \ref{prop:representation_f}]
% \textcolor{blue}{TK: Should be moved to Appendix, but didn't want to interfere with the files!}
% The first step is to replace first layer weights $A$ by $\hat A S_A$. This can be achieved
% by injecting the permutation $\pi_A$ in the first layer. Specifically we get
% \begin{align}
% \label{eq:repara_f_1}
% f(x) &= 1^\top \phi(B^\top \phi(A^\top x + \theta) + \tau) = 1^\top \phi(B^\top \pi_A \phi((A\pi_A)^\top x + \pi_A^\top \theta) + \tau) \\
% &=1^\top \phi((\pi_A^\top B)^\top \phi(S_A A^\top x + \pi_A^\top \theta) + \tau).
% \end{align}
% Next we need to replace the matrix $\pi_A^\top B$ using $V$ respectively $\hat V$. Let
% $n \in \bbR^{\Nouterlayer}$ be defined as $n_\ell = \N{AGb_\ell}^{-1}$, and $N = \diag(n)$. By definition
% we have $V = AGBN$, implying the relation $B =  G^{-1}A^{-1}V N^{-1}$. Using
% $A = \hat A S_A \pi_A^\top$, $V = \hat VS_V\pi_V^\top$, $S_A^{-1} = S_A$, and $\pi_A^{-1} = \pi_A^\top$, it follows that
% \begin{align*}
% \pi_A^\top B = \pi_A^\top G^{-1} \pi_A S_A \hat A^{-1} \hat V S_V \pi_V^\top N^{-1} = (\pi_A^\top G \pi_A)^{-1} S_A \hat A^{-1} \hat V S_V \pi_V^\top N^{-1}
% \end{align*}
% Now, since $G = \diag(\phi'(\theta))$, we have $\pi_A^\top G \pi_A = \diag(\pi_A^\top(\phi'(\theta))) = \diag(\phi'(\pi_A^\top\theta))=:\tilde G$.
% Inserting into \eqref{eq:repara_f_1}, we get
% \begin{align*}
% f(x) &=1^\top \phi(N^{-1} \pi_V S_V \hat V^\top \hat A^{-\top} S_A \tilde G^{-1} \phi(S_A A^\top x + \pi_A^\top \theta) + \tau)
% \end{align*}
% Furthermore, since the dot product with $1$ is permutation invariant, we can permute the activation of the second layer with $\pi_V^\top$. Then,
% using that $\tilde N = \pi_V^\top N \pi_V$ is diagonal, and thus commutes with $S_V$, we get
% \begin{align*}
% f(x) & =1^\top \phi(\tilde N S_V \hat V^\top \hat A^{-\top} S_A \tilde G^{-1} \phi(S_A A^\top x + \pi_A^\top \theta) + \pi_V^\top \tau) \\
% &= 1^\top \phi(\tilde N^{-1} S_V \hat V^\top \hat A^{-\top} S_A \tilde G^{-1} \phi(S_A A^\top x + \pi_A^\top \theta) + \pi_V^\top \tau)\\
% &= 1^\top \phi(S_V \tilde N^{-1}  \hat V^\top \hat A^{-\top} S_A \tilde G^{-1} \phi(S_A A^\top x + \pi_A^\top \theta) + \pi_V^\top \tau).
% \end{align*}
% It remains to show that $\hat B = \tilde G^{-1}  S_A \hat A^{-1} \hat V \tilde N^{-1}$, which is implied if $\tilde N$
% is a diagonal matrix with $\tilde N_{ll} = \Vert \tilde G S_A \hat A^{-1}\hat v_\ell\Vert$.
% Clearly $\tilde N$ is a diagonal matrix since $\tilde N = \pi_V^\top N \pi_V = \diag(\pi_V^\top n)$.
% Furthermore, the normalization $\N{b_\ell} = 1$ (see Definition \ref{def:f}) and $B =  G^{-1}A^{-1}V N^{-1}$ imply
% \begin{align*}
% 1 = \N{b_\ell} = \frac{\N{G^{-1}A^{-1}v_\ell}}{n_\ell}\quad \textrm{ and thus }\quad n_\ell = \N{G^{-1}A^{-1}v_\ell}.
% \end{align*}
% Using this, and $A^{-1} = \pi_A S_A \hat A^{-1}$, $V \pi_V = \hat V S_V$, we obtain
% \begin{align*}
% \tilde N &= \diag(\pi_V^\top n) = \diag\left(\pi_V^\top\left(\N{G^{-1}A^{-1}v_1},\ldots,\N{G^{-1}A^{-1}v_{\Nouterlayer}}\right)\right)\\
% &=\diag\left(\N{G^{-1}A^{-1}(V\pi_V)_1},\ldots,\N{G^{-1}A^{-1}(V\pi_V)_{\Nouterlayer}}\right)\\
% &=\diag\left(\N{G^{-1}\pi_A S_A \hat A^{-1}(\hat V S_V)_1},\ldots,\N{G^{-1}\pi_A S_A \hat A^{-1}(\hat V S_V)_{\Nouterlayer}}\right)\\
% &=\diag\left(\N{G^{-1}\pi_A S_A \hat A^{-1}\hat v_1},\ldots,\N{G^{-1}\pi_A S_A \hat A^{-1}\hat v_{\Nouterlayer}}\right),
% \end{align*}
% where we used that $S_V$ is only each column of $\hat V$ by $\pm 1$. The result follows since $\pi_A^\top$
% is orthogonal, so it can be inserted from the left into the norm, and we can replace $\pi_A^\top G^{-1}\pi_A = \tilde G^{-1}$.
% \end{proof}
% \begin{rem}[Simplification for odd functions]
% \label{rem:prop_simplification_odd_functions}
% If $\phi$ in Proposition \eqref{prop:representation_f} satisfies $\phi(-t) = -\phi(t)$,
% it is possible to show $\hat f(x; S S_A, S_V, S\pi_A^\top \theta, \pi_V^\top \tau) =
% f(x)$ for arbitrary sign matrix $S \in \CD_{\Ninnerlayer}$.
% \end{rem}
% %
% % \textcolor{red}{
% % TK: The following remark can be removed as it is `new' content, which I thought is interesting, but we haven't had time
% % to properly explore it. This allows
% % to set up an optimal program over $3\Ninnerlayer + 2\Nouterlayer$ variables,
% % which may be much easier to minimize and potentially has more stable gradients (no division by $S_A$)!
% % \begin{rem}[Different reparametrization]
% % \label{rem:different_network_reparametrization}
% % Assume again the setting of Proposition \ref{prop:representation_f}.
% % There exist diagonal matrices $D \in \CD_{\Nouterlayer}$ and $D \in \CD_{\Ninnerlayer}$ such that
% % \begin{align*}
% % f(x) = 1^\top\phi(D' \hat V^\top \hat A^{-T} D \phi(S_A \hat A^\top x + \pi_A^\top \theta) + \pi_V^\top \tau).
% % \end{align*}
% % In particular, denoting $\tilde G = \pi_A^\top G \pi_A = \diag(\phi'(\pi_A^\top\theta))$, optimal diagonal matrices are given by
% % \[
% % D' = S_V \diag\left(\N{\tilde G^{-1}S_A\hat A \hat v_1},\ldots,\N{\tilde G^{-1}S_A\hat A \hat v_{\Nouterlayer}}\right),\quad
% % D = \tilde G^{-1}S_A.
% % \]
% % \end{rem}
% % }
%
% \noindent
% Proposition \ref{prop:representation_f} implies that it suffices to correctly identify parameters
% $D, D', w, z$ in order to reconstruct a two layer
% network $\hat f$ which equals the original network function. This motivates to search
% for these parameters by minimizing the $L_2$-data fidelity of $\hat f$ with evaluations $Y_i=f(X_i)$
% over few additionally queried points $\{X_i : i \in [m_f]\}$, \emph{i.e.} to optimize the program
% \begin{equation}
% \label{eq:recover_network_functional}
% \min_{\substack{D \in \CD_{\Ninnerlayer}, D' \in \CD_{\Nouterlayer},\\ w \in \bbR^{\Ninnerlayer}, z \in \bbR^{\Nouterlayer}}}  J(D, D', w, z):=\sum_{i=1}^{m_f}\left(Y_i - \hat f(X_i;D, D', w, z)\right)^2.
% \end{equation}
% Assuming $\hat A$ and $\hat V$ are correct up to sign and permutation,
% Proposition \ref{prop:representation_f} implies that $J = 0$ is the global optimum,
% and it is attained by parameters leading to the original network $f$.
% Moreover, Remark \ref{rem:prop_simplification_odd_functions} implies that, if $\phi$ is an odd function,
% parameters $(S S_A, S_V, S^{-1} \pi_A^\top \theta, \pi_V^\top\tau)$ for arbitrary sign matrix $S$
% are also global optima that lead to the original function $f$.
%
%
% Compared to standard gradient descent methods for learning the complete network at once,
% functional \eqref{eq:recover_network_functional} has a signficantly reduced number of free
% parameters. This allows for fast computations, and additionally our numerical experiments below
% suggest that $m_f$ in the order of $\Ninnerlayer + \Nouterlayer$ suffice to reconstruct
% a good approximant to $f$. On the other hand, $J$ depends on the parameters $D$ and $w$
% in complicated manner so it is unclear how well the optimization problem is posed. In order to
% unerstand this better, we study
% the feasibility of \eqref{eq:recover_network_functional} with extensive  experiments below.
% We present results for the case when $\hat A$, and $\hat V$ are approximations computed using previously
% described methods, but also when $\hat A = A$ and $\hat V = V$.
%
% \begin{table}
% 	\begin{center}
% 		\begin{tabular}{ccccccc}
% 			\hline
% 			& \multicolumn{3}{c}{$\Ninnerlayer = 30$} & \multicolumn{3}{c}{$\Ninnerlayer = 45$}\\
% 			\hline
% 			Scenario & $\Nouterlayer =  3$ & $\Nouterlayer = 9$ & $\Nouterlayer = 15$ & $\Nouterlayer = 5$ & $\Nouterlayer = 14$ & $\Nouterlayer = 23$\\
% 			\hline
% 			& MSE,\ \  $E_{\infty}$ & MSE,\ \  $E_{\infty}$ & MSE,\ \  $E_{\infty}$ & MSE,\ \  $E_{\infty}$ & MSE,\ \  $E_{\infty}$ & MSE,\ \  $E_{\infty}$\\
% 			& Failed  & Failed  & Failed  & Failed  & Failed  & Failed  \\ \\ \hline
% 			POD/sig\\
% 			Pipeline & $0.9$, $7.8$ & $0.9$, $6.4$ & $9.5$, $27.8$ & $1.8$, $8.1$ & $1.1$, $6.3$ & $12.4$, $41.1$\\
% 			 & $17$ & $31$ & $45$ & $17$ & $10$ & $72$ \\
% 			$\hat A,\hat V = A,V$ & $<0.1$, $1.5$ & $0.2$, $2.0$ & $0.7$, $4.6$ & $<0.1$, $1.7$ & $0.2$, $2.2$ & $5.9$, $23.5$\\
%  			 & 0 & 0 & 3 & 0 & 0 & 0 \\ \\ \hline
% 			 POD/$\tanh$\\
%  			Pipeline & $11.1$, $52.3$ & $4.0$, $21.6$ & $1.1$, $12.0$ & $12.4$, $57.8$ & $4.3$, $18.5$ & $0.7$, $9.8$\\
%  			 & $53$ & $43$ & $13$ & $93$ & $30$ & $0$ \\
%  			$\hat A,\hat V = A,V$ & \multicolumn{6}{c}{All errors $<0.1$}\\
%   			 &  \multicolumn{6}{c}{ No failed cases} \\ \\ \hline
% 			$\bbS^{\Ninnerlayer - 1}$/sig\\
%  			% All & $12.5$, $56.0$ & $4.5$, $21.3$ & $1.7$, $14.2$ & $18.3$, $52.2$ & $0.8$, $10.1$ & $0.8$, $9.8$\\
%  			%  & $70$ & $57$ & $3$ & $93$ & $43$ & $0$ \\
%  			$\hat A,\hat V = A,V$ & $1.8$, $8.4$ & $0.8$, $8.2$ & $2.3$, $14.0$ & $0.5$, $5.5$ & $1.0$, $9.0$ & $2.2$, $16.0$\\
%   			 & $6$ & $0$ & $0$ & $0$ & $0$ & $3$ \\ \\
% 			\hline
% 			$\bbS^{\Ninnerlayer - 1}$/$\tanh$\\
%  			% All & $12.5$, $56.0$ & $4.5$, $21.3$ & $1.7$, $14.2$ & $18.3$, $52.2$ & $0.8$, $10.1$ & $0.8$, $9.8$\\
%  			%  & $70$ & $57$ & $3$ & $93$ & $43$ & $0$ \\
%  			$\hat A,\hat V = A,V$ & $<0.1$, $0.2$ & $1.1$, $3.5$ & $0.7$, $4$ & $<0.1$, $<0.1$ & $<0.1$, $<0.1$ & $<0.1$, $0.3$\\
%   			 & \multicolumn{6}{c}{ No failed cases} \\ \\ \hline
% 		\end{tabular}
% 	\end{center}
% 	\caption{Mean squared error (MSE) and $L_{\infty}$-error ($E_{\infty}$) of the reconstructed network using \eqref{eq:recover_network_functional}.
% 	All values represent percentages. We consider a trial as failed if $MSE > 20\%$. The scenarios correspond to those
% 	in Sections \ref{sec:numerical_NNprofiles} and \ref{subsec:distinguishing}. Pipeline indicates that we use $\hat A$ and $\hat V$
% 	by previously described methods. Otherwise we run \eqref{eq:recover_network_functional} with $A = \hat A$ and $V = \hat V$.}
% 	\label{tab:function_learning_results}
% \end{table}
%
%
% \begin{table}
% 	\begin{center}
% 		\begin{tabular}{ccccccc}
% 			\hline
% 			& \multicolumn{3}{c}{$\Ninnerlayer = 30$} & \multicolumn{3}{c}{$\Ninnerlayer = 45$}\\
% 			\hline
% 			Scenario & $\Nouterlayer =  3$ & $\Nouterlayer = 9$ & $\Nouterlayer = 15$ & $\Nouterlayer = 5$ & $\Nouterlayer = 14$ & $\Nouterlayer = 23$\\
% 			\hline
% 			& MSE,\ \  $E_{\infty}$ & MSE,\ \  $E_{\infty}$ & MSE,\ \  $E_{\infty}$ & MSE,\ \  $E_{\infty}$ & MSE,\ \  $E_{\infty}$ & MSE,\ \  $E_{\infty}$\\
% 			& Failed  & Failed  & Failed  & Failed  & Failed  & Failed  \\ \\ \hline
% 			POD/sig\\
% 			Pipeline & $1.2$, $7.9$ & $0.5$, $7.2$ & $1.2$, $11.7$ & $1.1$, $6.1$ & $0.3$, $6.0$ & $10.4$, $28.0$\\
% 			 & $24$ & $20$ & $17$ & $34$ & $10$ & $17$ \\
% 			$\hat A,\hat V = A,V$ & $<0.1$, $0.2$ & $<0.1$, $0.1$ & $<0.1$, $<0.1$ & $<0.1$, $0.2$ & $<0.1$, $<0.1$ & $1.8$, $11.1$\\
%  			 & \multicolumn{6}{c}{ No failed cases} \\ \\ \hline
% 			 POD/$\tanh$\\
%  			Pipeline & $-$, $-$ & $3.6$, $20.0$ & $2.0$, $15.8$ & $-$, $-$ & $3.0$, $18.1$ & $1.7$, $14.0$\\
%  			 & $100$ & $56$ & $13$ & $100$ & $40$ & $0$ \\
%  			$\hat A,\hat V = A,V$ & \multicolumn{6}{c}{All errors $<0.1$}\\
%   			 &  \multicolumn{6}{c}{ No failed cases} \\ \\ \hline
% 			$\bbS^{\Ninnerlayer - 1}$/sig\\
%  			% All & $12.5$, $56.0$ & $4.5$, $21.3$ & $1.7$, $14.2$ & $18.3$, $52.2$ & $0.8$, $10.1$ & $0.8$, $9.8$\\
%  			%  & $70$ & $57$ & $3$ & $93$ & $43$ & $0$ \\
%  			$\hat A,\hat V = A,V$ & $<0.1$, $0.3$ & $<0.1$, $0.1$ & $<0.1$, $<0.1$ & $<0.1$, $0.2$ & $<0.1$, $0.1$ & $1.3$, $10.7$\\
%   			 & \multicolumn{6}{c}{ No failed cases} \\ \\
% 			\hline
% 			$\bbS^{\Ninnerlayer - 1}$/$\tanh$\\
%  			% All & $12.5$, $56.0$ & $4.5$, $21.3$ & $1.7$, $14.2$ & $18.3$, $52.2$ & $0.8$, $10.1$ & $0.8$, $9.8$\\
%  			%  & $70$ & $57$ & $3$ & $93$ & $43$ & $0$ \\
%  			$\hat A,\hat V = A,V$ & \multicolumn{6}{c}{All errors $<0.1$}\\
%   			 & \multicolumn{6}{c}{ No failed cases} \\ \\ \hline
% 		\end{tabular}
% 	\end{center}
% 	\caption{Mean squared error (MSE) and $L_{\infty}$-error ($E_{\infty}$) of the reconstructed network using \eqref{eq:recover_network_functional}
% 	while fixing $D = \Id_{\Ninnerlayer}$. For description of the Table see \ref{tab:function_learning_results}.}
% 	\label{tab:function_learning_results_woSa}
% \end{table}
%
%
% \paragraph{Numerical experiments}
% We minimize \eqref{eq:recover_network_functional} with standard gradient descent and
% learning rate $1$ if $\phi(t) = \frac{1}{1+e^{-t}} - 1/2$ (shifted sigmoid),
% and learning rate $0.025$ if $\phi(t) = \tanh(t)$. We sample $m_f = 10(\Ninnerlayer + \Nouterlayer)$
% additional points according to $X_i \sim \CN(0,\Id_{\Ninnerlayer})$.
% Moreover, gradient descent is run for 500K iterations (due to small number of variables,
% this is not time consuming), and only prematurely stopped if the iteration stalls. All variables
% are initialized with draws from $\CN(0,0.1)$.
%
% Denoting $S_A^*, S_V^*, \theta^*, \tau^*$ as the gradient descent output, we assess the feasibility
% of \eqref{eq:recover_network_functional} by the relative mean squared error (MSE) and the relative $L_{\infty}$-error
% \[
% \textrm{MSE} = \frac{\sum_{i=1}^{m_{\textrm{test}}}\hat f(Z_i;S_A^*, S_V^*, \theta^*, \tau^*) - f(Z_i))^2}{\sum_{i=1}^{m_{\textrm{test}}}f(Z_i)^2},\quad
% \textrm{E}_{\infty} = \frac{\max_{i \in [m_{\textrm{test}}]}\SN{f(Z_i;S_A^*, S_V^*, \theta^*, \tau^*) - f(Z_i)}}{\max_{i \in [m_{\textrm{test}}]}\SN{f(Z_i)}},
% \]
% using $m_{\textrm{test}} = 50000$ samples $Z_i \sim \CN(0,\Id_{\Ninnerlayer})$.
%
%
% We repeat each experiments 30
% times, and classify all trials where MSE$> 0.2$ as failed.
% With few exceptions, in these cases matrices $\hat A$ and $\hat V$ are poor approximations
% to $A$ and $V$ such the minimization of \eqref{eq:recover_network_functional} does not
% provide a good approximation of $f$. The results over all remaining trials are averaged
% and reported, alongside the percentage of failed tries.
%
% Table \ref{tab:function_learning_results} summarizes the results of the study. For
% the cases $\hat A = A$ and $\hat V = V$, minimizing \eqref{eq:recover_network_functional}
% with $m_f = 10(\Ninnerlayer + \Nouterlayer)$ additional points achieves convincing
% performance since both the $L_2$-error and $L_{\infty}$-error become small. In many of
% these trials, the errors are actually close to machine precision, or can be driven that far
% by using additional GD-iterations, or higher learning rates. This suggests that the minimization
% indeed recovers the original network function. On the other hand, Table \ref{tab:function_learning_results} also shows that
% \eqref{eq:recover_network_functional} is quite sensitive towards $\hat A$ and $\hat V$ because the
% number of failed trials increases significantly if we instead use approximated $\hat A$ and $\hat V$.
% It is also in accordance with results of Sections \ref{sec:numerical_NNprofiles}
% and \ref{subsec:distinguishing} that learning the function is easier for $\tanh$ activation
% (sigmoid activation) if $m_1$ increases (decreases).
%
% We also tested \eqref{eq:recover_network_functional} when fixing $D = \Id_{\Ninnerlayer}$
% since both activation functions we test are odd functions, and thus Remark \ref{rem:prop_simplification_odd_functions}
% applies. Table \ref{tab:function_learning_results_woSa} shows that this further
% improves the performance when using $\hat A = A$ and $\hat V = V$,
% but can have detrimental effect in the approximate cases.

